Distributed Download from an External Data Source in Faulty Majority Settings

We extend the study of retrieval problems in distributed networks, focusing on improving the efficiency and resilience of protocols in the \emph{Data Retrieval (DR) Model}. The DR Model consists of a complete network (i.e., a clique) with $k$ peers, up to $\beta k$ of which may be Byzantine (for $\beta \in [0, 1)$), and a trusted \emph{External Data Source} comprising an array $X$ of $n$ bits ($n \gg k$) that the peers can query. Additionally, the peers can also send messages to each other. In this work, we focus on the Download problem that requires all peers to learn $X$. Our primary goal is to minimize the maximum number of queries made by any honest peer and additionally optimize time. We begin with a randomized algorithm for the Download problem that achieves optimal query complexity up to a logarithmic factor. For the stronger dynamic adversary that can change the set of Byzantine peers from one round to the next, we achieve the optimal time complexity in peer-to-peer communication but with larger messages. In broadcast communication where all peers (including Byzantine peers) are required to send the same message to all peers, with larger messages, we achieve almost optimal time and query complexities for a dynamic adversary. Finally, in a more relaxed crash fault model, where peers stop responding after crashing, we address the Download problem in both synchronous and asynchronous settings. Using a deterministic protocol, we obtain nearly optimal results for both query complexity and message sizes in these scenarios.

==> Crash_Faults/asynchronous.tex <==
\section{The Asynchronous Data Retrieval Model with Crash Faults} \label{sec:async_crash_faults}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Download with At Most One Crash}

We start the exploration of the asynchronous setting with an algorithm that solves Download with at most one crash fault. This serves as an introduction for our main algorithm, handling an arbitrary number of crashes.

The algorithm runs in two phases. In each phase, every \peer maintains a list of assigned indices. Each phase has three stages, and every message contains the local phase number and stage number. We describe a single phase and particularly the operation of \peer $M_i$.

In stage 1, the \peer $M_i$ queries all assigned bits that are still unknown and sends stage-1 messages containing the assigned bits' values to all other \peers. (Assuming it is necessary to send the assigned bits in multiple packets, each packet would also include the packet number.) 

In stage 2, every \peer $M_i$ waits until it receives all stage-1 messages (according to its local assignment) from at least $k-1$ \peers (waiting for the last {\peer} risks deadlock, in case that {\peer} has crashed). When that condition is met, $M_i$ sends a stage-2 message containing the index $j$ of the \emph{missing} \peer, namely, the \peer $M_j$ from which it didn't receive all stage-1 messages during the current phase. When $M_i$ receives a stage-2 message containing the index $j$, it sends a stage-2 response containing either the bits assigned to $M_j$ (if it heard from $M_j$) or \metoo\ if it didn't hear from $M_j$ during stage 2. (In case $M_i$ hasn't finished waiting for stage-1 messages, it delays its response until it is finished.)

Finally, in stage 3, every \peer $M_i$ waits until it collects at least $k-1$ stage-2 responses. When that happens, there are two cases. Either $M_i$ has received only \metoo\ messages, in which case it reassigns the bits of $M_j$ evenly to all \peers and starts the next phase, or $M_i$ has received $M_j$'s bits from at least one \peer, in which case it goes into \textit{completion} mode, which means that in the next phase, $M_i$ acts as follows. In stage-1, it sends all the bits in stage-1 messages. In stage-2, it doesn't send stage-2 messages, and in stage-3, it doesn't wait for stage-2 responses.

After two phases, every \peer terminates.

Note that if a \peer receives a message from (another {\peer} which is in) a later phase, it stores it for future use, and if it receives a message from an earlier phase, it retrieves the bits the message (possibly) holds and evaluates whether or not to enter completion mode 

See Algorithm \ref{alg:single_crash_async_down} for the formal code.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
    \caption{Asynchronous Download one crash (code for \peer $M_i$)} \label{alg:single_crash_async_down}
    \begin{algorithmic}[1]
    \State $Mode \gets$ Active
    \For{$t \in \{1, 2\}$}
        \Procedure{Stage 1}{}
        \State Query all unknown assigned bits.
        \If{$Mode =$ Active}
            \State Send a stage-1 message with the assigned bits to every other \peer. 
        \Else
            \State Send a stage-1 message with all known bits.

        \EndIf

        \State (In the CONGEST model, this message may need to be broken into packets of size $O(\log n)$.)
    \EndProcedure
    \Procedure{Stage 2}{}
        \State Maintain the following set:
        \Statex $H = \{j \mid \text{received all stage-1 messages from } M_j \}$
        \State When $|H| \geq k-1$, if $Mode=$Active, send $J_f(i)$ s.t. $\{J_f(i)\} = \{1, \dots, k\} \setminus H$ to all other \peers. 
        \State  \textbf{When}
        % \hl{If statement is required}
        receiving a stage-2 message $J_f(i')$ from \peer $M_{i'}$:
        \Statex Send back a stage-2 response containing \metoo\ if $J_f(i') = J_f(i)$ and $M_{J_f(i')}$'s assigned bits otherwise. 
    \EndProcedure
    \Procedure{Stage 3}{}
        \If{$Mode=$Active}
        \State Collect stage-2 responses until receiving at least $k-1$ messages.
        \If{Received only \metoo\ responses}
            \State Reassign $M_{J_f(i)}$'s bits to \peers $I =\{1, \dots, k \} \setminus \{J_f(i)\}$, and start the next phase. 
        \Else
            \State $Mode \gets$ completion
        \EndIf
        \EndIf
    \EndProcedure
    \Procedure{messages from different phases}{}
        \If{
        Received a message from a different phase}
            \State If it is from a later phase, store it for future use.
            \Statex If it is from a previous phase, evaluate its content and update your known bits accordingly. If you have no more unknown bits, go into completion mode. 
        \EndIf
    \EndProcedure
    \EndFor
    \end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We use the following facts to show the correctness and compelxity of the protocol.

\begin{observation} \label{obs:overlap}
    (Overlap Lemma) Assuming $2f<k$, every two sets of $k-f$ \peers must overlap at least one \peer.
\end{observation}
\begin{proof}
%This follows since 
Exactly $f$ distinct \peers are not present in one of the sets, hence at least $k-2f \geq 1$ \peers in the other set must not be distinct, thereby being in both sets.
\end{proof}

The following observation holds after each of the two phases, although a stronger property holds after phase 2, namely, each \nonfaulty \peer knows all input bits.

\begin{observation} \label{obs:peers_missing}
After Stage 2, every \peer lacks bits from at most one ``missing" \peer.
\end{observation}

This observation is obvious from the algorithm since each \peer receives all stage-1 messages from at least $k-1$ \peers.

\begin{lemma} \label{lem:stage_3_uniquness}
After stage 3, if two different \peers $M_i$ and $M_{i'}$ lack bits from missing \peers $M_j$ and $M_{j'}$ respectively, then $j=j'$.
\end{lemma}

\begin{proof}
Let $M_i$ and $M_{i'}$ be \peers as required by the premises of the lemma. $M_i$ received $k-1$ \metoo\ messages for $j$ and $M_{i'}$ received $k-1$ \metoo\ messages for $j'$. By the Overlap Lemma \ref{obs:overlap}, there is at least one \peer that sent \metoo\ to both $M_i$ and $M_{i'}$ for $j$ and $j'$ respectively, yet, by Observation \ref{obs:peers_missing}, each \peer lacks bits from at most one missing \peer. Hence, $j=j'$.
\end{proof}

\begin{theorem} \label{thm:async_single_crash}
% Algorithm \ref{alg:single_crash_async_down}, solves \IDp\ in the asynchronous setting with at most one crash fault after 2 phases with $\Query = n/k + n/k(k-1)$.
In the asynchronous model with $1$ crash fault, there is a deterministic protocol that solves Download with $\Query =\frac{n}{k} + \lceil\frac{n}{k(k-1)}\rceil$, $\Time = \tilde{O}\left(\frac{n}{k}\right)$ and $\Message = O(nk)$.

\end{theorem}
\begin{proof}
By Observation \ref{obs:peers_missing}, after stage 2 of phase 1, each \peer $M_i$ lacks bits from at most one missing \peer. By Lemma \ref{lem:stage_3_uniquness}, after stage 3 of phase 1, every \peer $M_i$ that still lacks some bits has the same missing \peer $M_j$. Consider such a \peer $M_i$. At the end of stage 3 of phase 1, $M_i$ reassigns the bits of $M_j$ evenly to $I =\{1, \dots, k\} \setminus \{j\}$. Every \peer in $I$ either lacks some bits from $M_j$ or is in completion mode, so in the following phase 2, they will send stage-1 messages consistent with the local assignment of $M_i$. Hence, in stage 2 of phase 2, either $M_i$ receives a phase-2 stage-1 message from $M_j$, meaning it also receives a phase-1 stage-1 message from $M_j$, or it receives all phase-2 stage-1 messages from all \peers in $I$. In both cases, there are no unknown bits after stage 2 of phase 2.

In terms of query complexity, each \peer queries $n/k$ times in phase 1. Because each \peer lacks bits from at most one \peer, it has at most $n/k$ unknown bits. At the end of stage 3 of phase 1, every such \peer reassigns those $n/k$ bits evenly to the remaining $k-1$ \peers, resulting in additional $n/(k(k-1))$ queries per \peer. In total, the query complexity is $n/k + n/(k(k-1))$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Extending the Result to \texorpdfstring{$f$}{} Crashes}
    In this subsection, we present a protocol that extends Algorithm \ref{alg:single_crash_async_down} to an algorithm that can tolerate up to $f$ crashes for any $f<k$.
    
    The main difficulty in achieving tolerance with up to $f$ crashes is
    that in the presence of asynchrony, one cannot distinguish between a slow \peer and a crashed \peer,
    making it difficult to coordinate.
    
    Similarly to Algorithm \ref{alg:single_crash_async_down}, Algorithm \ref{alg:f_crash_async_down} executes in phases, each consisting of three stages. Each \peer $M$ stores the following local variables.
    \begin{itemize}
        \item $phase(M)$: $M$'s current phase.
        \item $stage(M)$: $M$'s current stage within the phase.
        \item $H_p^M$: the \emph{correct set} of $M$ for phase $p$, i.e., the set of \peers $M$ heard from during phase $p$.
        \item $\sigma_p^M$: the \emph{assignment function} of $M$ for phase $p$, which assigns the responsibility for querying each bit $i$ to some \peer $M'$.
        \item $\res^M$: the output array.
    \end{itemize}
    We omit the superscript $M$ when it is clear from the context.
    
    In the first stage of phase $p$, each \peer $M$ queries bits according to its local assignment $\sigma_p$ and sends a $\phase \ p \ \stage \ 1$ request (asking for bit values according to $\sigma_p$, namely $\{i \mid \sigma_p(i) = M'\}$) to every other \peer $M'$ and then continues to stage 2.
    Upon receiving a $\phase \ p \ \stage \ 1$ request, $M$ waits until it is at least in stage 2 of phase $p$ and returns the requested bit values that it knows.
    In stage 2 of phase $p$, $M$ waits until it hears from at least $|H_p^M| \geq k-f$ \peers (again, waiting for the remaining $f$ {\peers} risks deadlock). Then, it sends a $\phase \ p \ \stage \ 2$ request containing the set of \peer Id's $F_p^M = \{1, \dots, k\}\setminus H_p^M$ (namely, all the \peers it didn't hear from during phase $p$) and continues to stage 3.
    Upon receiving a $\phase \ p \ \stage \ 2$ request, $M$ waits until it is at least in stage 3 of phase $p$, and replies to every \peer $M'$ as follows. For every $j\in F_p^{M'}$, it sends $M_j$'s bits if $j\in H_p^{M'}$ and \metoo\ otherwise.
    In stage 3 of phase $p$, $M$ waits for $k-f$ $\phase \ p \ \stage \ 2$ responses. Then, for every $j\in F_p^M$, if it received only \metoo\ messages, it reassigns $M_j$'s bits evenly between \peers $1, \dots, k$. Otherwise, it updates $\res$ in the appropriate indices. Finally, it continues to stage 1 of phase $p+1$.
    Upon receiving a $\phase \ p \ \stage \ i$ response, $M$ updates $\res$ in the appropriate index and updates $H_p$ for every bit value in the message. See Algorithm \ref{alg:f_crash_async_down} for the formal code.

    Before diving into the analysis, we overview the following intuitive flow of the algorithm's execution. At the beginning of phase 1, the assignment function $\sigma_1$ is the same for every \peer. Every \peer is assigned $n/k$ bits, which it queries and sends to every other \peer. Every \peer $M$ hears from at least $k-f$ \peers, meaning that it has at most $f\cdot n/k$ unknown bits after phase 1. In the following phases, every \peer $M$ reassigns its unknown bits uniformly among all the \peers, such that the bits assigned to every \peer $M'$ are either known to it from a previous phase or $M'$ is about to query them in the current phase (i.e., $M'$ assigned itself the same bits). Hence, after every phase, the number of unknown bits diminishes by a factor of $f/k$. After sufficiently many phases, the number of unknown bits will be small enough to be directly queried by every \peer.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
    \caption{Async Download version 2 for \peer $M$} \label{alg:f_crash_async_down}
    \begin{algorithmic}[1]
    
    
    \State \textbf{Local variables} 

    \State $phase(M)$, initially 0 \Comment{This is the present phase of $M$}

    \State $stage(M)$, initially 1 \Comment{This is the present stage of $M$}

    \State $H_p$, $p \in \mathbb{N}$, initially $\emptyset$      \Comment{The set of \peers $M$ heard from during phase $p$}
    \State $\sigma_p(i)$, $p \in \mathbb{N}$, initially $\sigma_p(i) \gets M_{1+\lceil i / \frac{n}{k}\rceil}$  \Comment{The assignment function of $M$ in phase $p$}
    \State $\res[i]$, $i\in \{1,\dots, n\}$, initially $\bot$ \Comment{Output array}

    \State 

    \Upon{entering stage 1 of phase $p$}
        \State \Comment{--------- stage 1 (start) ---------------------------------}
        \State Query all unknown assigned bits, $\{i \mid \res[i]=\bot, \sigma_p(i) = M\}$.
        \State Send a $\phase \ p \ \stage \ 1$ request containing $\{i \mid \res[i] = \bot, \sigma_p(i) = M'\}$ to every \peer
        % $M'$ 
        \State Set $stage(M)\gets 2$
        % \State \Comment{--------- stage 1 (end) ---------------------------------}

        \State \Comment{--------- stage 2 (start) ---------------------------------}
        \State Wait until $|H_p| \geq k-f$ \label{line:wait_2} 
        \State  Send a $\phase\ p\ \stage\ 2$ request containing $F_p=\{1,\dots, k\}\setminus H_p$ to every \peer $M'$ 
        \State Set $stage(M)\gets 3$
        \State \Comment{--------- stage 3 (start) ---------------------------------}
        \State Wait until received at least $k-f$ $\phase$ $p$ $\stage$ $2$ responses.\label{line:wait_3} 
        \For{$j \in F_p$} 
            % \State Wait until received at least $k-f$ $\phase$ $p$ $\stage$ $2$ responses.\label{line:wait_3}
            \If{Received only \metoo\ responses for $j$}
                \State Let $i_0, \dots, i_{n'-1}$ be the indices such that $\sigma(i_l) = M_j$, $0\leq l\leq n'-1 $.
                \State Set $\sigma_{p+1}(i_l) \gets M_{1+\lceil l / \frac{n'}{k} \rceil}$, $0\leq l\leq n'-1 $.\label{line:reassign}
                \Comment{ Reassign $M_j$'s bits to all $\{1, \dots, k \}$} 
            \Else
                \For{$i \in \{i \mid \sigma(i) = M_j\}$}
                    \State $\res[i] \gets b_i$
                \EndFor
                \Comment{Update $\res$ in the appropriate indices}
                % \State $Mode \gets$ completion
            \EndIf
        \EndFor
        \State Set $phase(M)\gets phase(M)+1$, $stage(M)\gets 1$ 
        
        % , $<\mathtt{p}, \mathtt{request\text{-}1}, \{i \mid,\sigma(i) = M'\}>$
    \EndUpon
    
    \State
    
    \Upon{seeing a $\phase \ p \ \stage \ 1$ request for bit Set $B$}
        \State Store the request until $phase(M)=p$ and $stage(M)\geq 2$ or $phase(M) >p$ 

        \State Send back a $\phase \ p \ \stage \ 1$ response containing $\{\langle i, \res[i] \rangle \mid i \in B\}$
        
        % \If{$B \subseteq \{i\mid \res[i] \neq \bot\} $}
        %     \State Send a $\phase \ p \ \stage \ 1$ response containing $\{\langle i, \res[i] \rangle \mid i \in B\}$
        % \Else
        %     \State Send "$x$".
        % \EndIf
    \EndUpon

    \State

    \Upon{seeing a $\phase \ p \ \stage \ 2$ request containing $F$ from $M'$}{}
        \State  Store the request until $phase(M)=p$ and $stage(M)\geq 3$ or $phase(M) >p$ 
        \For{$j \in F_p$}
            \State  Send back a $\phase\ p \ \stage \ 2$ response containing \metoo\ if $j\notin H_p$ and $M_j$'s assigned bits otherwise.
        \EndFor  
    \EndUpon

    \State
    \Upon{receiving a $\phase \ p$ $\stage \ i$ response}{}
        \State For every bit value in the message $\langle i, b_i \rangle$, set $\res[i] \gets b_i$
        \State Update $H_p \gets \{j \mid \res[i]\neq \bot \ \ \forall i :\sigma_p(i) = j\}$
        % \If{$phase(M) == p$ }
        %     \State Update $H_p = \{j \mid \res[i]\neq \bot \ \forall i :\sigma(i) = j\}$
        % \ElsIf{$phase(M) > p$}
        %     \State 
        % \Else
        % \EndIf
    \EndUpon
    \State 
    
    % \Procedure{entering stage 2 of phase $p$}{}
    %     \State Wait until $|H_p| \geq k-f$ \label{line:wait_2}
    %     \State  Send a $\phase\ p\ \stage\ 2$ request containing $F_p=\{1,\dots, k\}\setminus H_p$ to every \peer $M'$ 
    %     \State Set $stage(M)\gets 3$
    % \EndProcedure

    
    

    % \State 

    % \Procedure{entering stage 3 of phase $p$}{}
        % \State Wait until received at least $k-f$ $\phase$ $p$ $\stage$ $2$ responses.\label{line:wait_3}
        % \For{$j \in F_p$}
        %     \State Wait until received at least $k-f$ $\phase$ $p$ $\stage$ $2$ responses.\label{line:wait_3}
        %     \If{Received only \metoo\ responses for $j$}
        %         \State Let $i_0, \dots, i_{n'-1}$ be the indices such that $\sigma(i_l) = M_j$ $0\leq l\leq n'-1 $.
        %         \State Set $\sigma_{p+1}(i_l) \gets M_{\lceil l / \frac{n'}{k} \rceil}$, $0\leq l\leq n'-1 $.\label{line:reassign}
        %         \Comment{ Reassign $M_j$'s bits to all $\{0, \dots, k-1 \}$} 
        %     \Else
        %         \For{$i \in \{i \mid \sigma(i) = M_j\}$}
        %             \State $\res[i] \gets b_i$
        %         \EndFor
        %         \Comment{Update $\res$ in the appropriate indices}
        %         % \State $Mode \gets$ completion
        %     \EndIf
        % \EndFor
        % \State Set $phase(M)\getsphase(M)+1$, $stage(M)\gets1$
    % \EndProcedure

    % \State 
    \Upon{$phase(M) = \log_{k/f}(n)$ or $H_p=\{1, \dots, k\}$}{}
    \label{line:termination_condition}
    \State Query all unknown bits
        \State Send $\res$ to every other \peer and Terminate
    \EndUpon
    
    % \If{$phase(M) = \log_{k/f}(n)$ or $H_p=\{0, \dots, k-1\}$} 
    %     \State Query all unknown bits
    %     \State Send $\res$ to every other \peer and Terminate
    % \EndIf
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We start the analysis by showing some properties on the relations between local variables.
\begin{observation} \label{obs:no_missing_mahines_no_missing_bits}
    For every \nonfaulty \peer $M$, if $H_p^M=\{1, \dots, k\}$ for some phase $p\geq 0$ then $\res^M=\invec$
\end{observation}
\begin{proof}
    Let $p\geq 0$ be such that $H_p=\{1, \dots, k\}$,
    and consider $1\leq i\leq n$. There exists some $1\leq j\leq k$ such that $\sigma_p(i) = M_j$. Since $j \in H_p^M$, $M$ has heard from $M_j$, so $\res^M[i] \neq \bot$, and overall $\res^M=\invec$.
\end{proof}

Denote by $\sigma^M_p$ the local value of $\sigma_p$ for \peer $M$ at the beginning of phase $p$.
Denote by $\res^M_p[i]$ the local value of $\res[i]$ for \peer $M$ after stage 1 of phase $p$.


\begin{claim} \label{claim:matching_assignment}
For every phase $p$, two \nonfaulty \peers $M, M'$, and bit $i$, one of the following holds.
\begin{enumerate}[$(1_p)$]
    \item $\sigma^M_p(i) =\sigma^{M'}_p(i)$, i.e., both $M$ and $M'$ assign the task of querying $i$ to the same \peer, or
    \item $\res^M_p[i] \neq \bot$ or $\res^{M'}_p[i] \neq \bot$. 
\end{enumerate}
\end{claim}
\begin{proof}
By induction on $p$.
For the basis, $p=0$, the claim is trivially true because of the initialization values (specifically, 
%claim
property ($1_0$) holds).

For $p\geq 1$. By the induction hypothesis, either $(1_{p-1})$ or $(2_{p-1})$ holds. 
Suppose first that $(2_{p-1})$ holds, i.e., $\res^M_{p-1}[i] \neq \bot$ or $\res^{M'}_{p-1}[i] \neq \bot$. Without loss of generality, assume that $\res^M_{p-1}[i] \neq \bot$. Then, since values are never overwritten, $\res^M_p[i] \neq \bot$, so $(2_p)$ holds as well.

Now suppose that $(1_{p-1})$ holds, i.e., $\sigma^M_{p-1}(i) =\sigma^{M'}_{p-1}(i)$. Let $j$ be an index such that $\sigma^M_{p-1}(i)=M_j$. If both $M$ and $M'$ didn't hear from $M_j$ during phase $p-1$, then both \peers will assign the same \peer to $i$ in stage 3 of phase $p-1$ (see Line \ref{line:reassign}), so $(1_p)$ holds. If one of the \peers heard from $M_j$, w.l.o.g assume $M$ did, then $\res^M_p[i] \neq \bot$. Hence, $(2_p)$ holds.
\end{proof}

Claim \ref{claim:matching_assignment} yields the following corollary.

\begin{corollary} \label{cor:correct_response}
    Every phase $p$\ stage $1$ request received by a \nonfaulty \peer is answered with the correct bit values.
\end{corollary}

Next, we show that the algorithm never deadlocks, i.e., whenever a \nonfaulty \peer waits in stages 2 and 3 (see Lines \ref{line:wait_2} and \ref{line:wait_3}), it will eventually continue.

\begin{claim} \label{claim:one_nonfaulty_termination}
    If one \nonfaulty \peer has terminated, then every \nonfaulty \peer will eventually terminate.
\end{claim}
\begin{proof}
    Let $M$ be a \nonfaulty \peer that has terminated. Prior to terminating, $M$ queried all the remaining unknown bits and sent all of the bits to every other \peer. Since $M$ is \nonfaulty, every other \nonfaulty \peer $M'$ will eventually receive the message sent by $M$ and will set $H_p^{M'} = \{1, \dots, k\}$, resulting in $\res^{M'}=\invec$ by Observation \ref{obs:no_missing_mahines_no_missing_bits}. Subsequently, $M'$ will terminate as well.
\end{proof}
\begin{claim} \label{claim:finite_wait}
    While no \nonfaulty \peer has terminated, a \nonfaulty \peer will not wait infinitely for $k-f$ responses.
\end{claim}
\begin{proof}
    First, note that at least $k-f$ \peers are \nonfaulty and by Corollary \ref{cor:correct_response} will eventually respond if they see a request before they terminate. Thus, the only case in which a \peer will not get $k-f$ responses is if at least one \nonfaulty \peer has terminated. 
\end{proof}

The combination of Claims \ref{claim:finite_wait} and \ref{claim:one_nonfaulty_termination} implies that eventually, every \nonfaulty \peer satisfies the termination condition (see Line \ref{line:termination_condition}) and subsequently terminates correctly (since it queries all unknown bits beforehand). That is because by Claim \ref{claim:finite_wait} some \nonfaulty \peer $M$ will get to phase $\log_{k/f}(n)$, or set $H_p^M=\{1, \dots, k\}$ prior to that, and terminate, which will lead to the termination of every \nonfaulty \peer by Claim \ref{claim:one_nonfaulty_termination}.



% Yet, in that case, the terminated \nonfaulty \peer has downloaded all unknown bits (so it stores the entire input) and sent $\res$ to all \peers, which means that eventually, every \nonfaulty \peer will set $H_p=\{0, \dots, k-1\}$ and terminate.


\begin{claim} \label{claim:unkown_bits_per_phase}
    At the beginning of phase $p\geq 0$, every \nonfaulty \peer has at most $n\cdot \left(\frac{f}{k}\right)^p$ unknown bits.
    % and $\frac{n}{k}\cdot (\frac{f}{k})^p$ unknown assigned bits.
\end{claim}
\begin{proof}
    By induction on $p$. Consider \nonfaulty \peer $M$.
    %
    For the base step $p=0$ the claim holds trivially by the initialization values.
    
    Now consider $p\geq 1$.
    By the induction hypothesis on $p-1$, $M$ has at most $\hat{n} = n\cdot \left(\frac{f}{k}\right)^{p-1}$ unknown bits at the start of phase $p-1$.
    Since unknown bits are assigned evenly in stage $3$ (see Line \ref{line:reassign}), each \peer is assigned $\hat{n}/k$ unknown bits (to be queried during phase $p-1$).
    During stage 2 of phase $p-1$, $M$ waits until $|H_{p-1}^M| \geq k-f$, meaning that $M$ did not receive the assigned bits from at most $f$ \peers.
    % Since unknown bits are assigned evenly in stage $3$ (see Line \ref{line:reassign}), each \peer is assigned $\hat{n}/k$ unknown bits for every \peer that didn't sent a stage 2 phase $p-1$ response during phase $p-1$ .
    Hence, there are at most $\hat{n}/k \cdot f = n\cdot \left(\frac{f}{k}\right)^p$ unknown bits after stage 2 of phase $p$. The claim follows.
\end{proof}

By Claim \ref{claim:unkown_bits_per_phase} and since unknown bits are distributed evenly among $\{0, \dots, k-1\}$, every \nonfaulty \peer queries at most $\frac{n}{k}\cdot \left(\frac{f}{k}\right)^{p}$ in phase $0\leq p\leq \log_{k/f}(n)$ and at most $\frac{n}{k}\cdot \left(\frac{f}{k}\right)^{\log_{k/f}(n)} = \frac{1}{k}$ additional bits when terminating (By Observation \ref{obs:no_missing_mahines_no_missing_bits}). Hence, the worst case query complexity (per \peer) is bounded by 
$$\Query ~\leq~ \frac{1}{k} + \sum_{p=1}^{\log_{k/f}(n)} \frac{n}{k}\cdot \left(\frac{f}{k}\right)^{p} ~=~ O\left(\frac{n}{\goodfrac k}\right).$$
%queries.

We next turn to time analysis.
%Note that for the same reasons, 
% Let $f_p$ be the number of {\peers} that crashed during phase $p$. We observe that in subsequent phases $p'>p$, none of the {\peers} heard from at least $f_p$ {\peers} which results in \say{me too} responses for $f_p$ out of $f$ {\peers} that were not heard during phase $p$.
Let $M$ be a \peer. For every phase $p$, after $n/k \cdot (\frac{f}{k})^p$ time, every $\phase\ p\ \stage\ 1$ response by a \nonfaulty {\peer} is heard by $M$ (even slow ones),
and stage 2 starts. After that, it takes at most $n \cdot (\frac{f}{k})^{p+1}$ time units for every $\phase\ p\ \stage\ 2$ response to be heard by $M$, allowing it to move to stage 3. Hence, it takes at most $n/k \cdot (\frac{f}{k})^p + n \cdot (\frac{f}{k})^{p+1}$ time for phase $p$ to finish once $M$ started it. Finally, upon termination, $M$ sends $\res_M$ which takes $n$ time. Overall the time complexity is 

\[
\Time ~\le~ n + \sum_{p=0}^{\log_{k/f}(n)} \left(\frac{n}{k} \cdot \left(\frac{f}{k}\right)^p + n \cdot \left(\frac{f}{k}\right)^{p+1}\right) ~=~ n + O\left(\frac{n\cdot f}{\goodfrac k}\right) ~=~ O\left(\frac{\byzfrac}{\goodfrac}\cdot n\right).
\]

This results in the following.
\begin{lemma}
Algorithm \ref{alg:f_crash_async_down} solves Download in the asynchronous setting with at most $f$ crash faults after $\log_{k/f}(n)$ phases with $\Query = O(\frac{n}{\goodfrac k})$ and $\Time = n + O(\frac{\byzfrac}{\goodfrac}\cdot n)$.
\end{lemma}


The following explains how we get better time complexity 
Note that this requires a slight modification of the code.
To make the time complexity analysis more precise, we identify a necessary condition for a \peer to send bits in a $\phase\ p \ \stage\ 2$ response (rather than %\say{me too}
\metoo). We observe that after 1 time unit, every message is delivered (even by slow \peers). Hence, after at most $\frac{n}{k}\cdot \left(\frac{f}{k}\right)^{p}$ time units, every $\phase\ p\ \stage\ 1$ response that was sent is delivered (including slow ones).
Therefore, while waiting for $k-f$ $\phase\ p\ \stage\ 2$ responses, it might be the case that a slow $\phase\ p\ \stage\ 1$ response arrives from \peer $M'$ eliminating the need for $\phase\ p\ \stage\ 2$ responses regarding \peer $M'$. 
The modification needed for this argument to work is that if $\phase\ p\ \stage\ 2$ responses regarding \peer $M'$ are no longer necessary because of its $\phase\ p\ \stage\ 1$ response arriving, $M$ is not blocked from continuing. Note that it is easy to see that this modification doesn't effect the correctness of the protocol.
Hence, the only time when a \peer must wait for a long $\phase\ p\ \stage\ 2$ response is when the corresponding \peer for which a $\phase\ p\ \stage\ 1$ response was not received has crashed (and therefore its $\phase\ p\ \stage\ 1$ response will never arrive). Also note that once a \peer crashed in phase $p$, it will not be heard from by any \peer in following phases resulting in 
%\say{me too} 
\metoo\
responses. Therefore every \peer waits for long $\phase\ p\ \stage\ 2$ responses at most $f$ times.
This results in the complexity being
\[\Time ~\leq~ n + \beta n + \sum_{p=0}^{\log_{k/f}(n)} \frac{n}{k} \cdot \left(\frac{f}{k}\right)^p ~=~ O\left(n + \frac{n}{\goodfrac k}\right) ~=~ O(n) .
\]
%david{So it is simply $O(n)$.}

\begin{theorem} \label{thm:async_multi_crash}
%Algorithm \ref{alg:f_crash_async_down} 
There is a deterministic algorithm for solving Download in the asynchronous setting with at most $f$ crash faults 
%after $\log_{k/f}(n)$ phases
with $\Query = O(\frac{n}{\goodfrac k})$ and $\Time = O(n)$.
\end{theorem}


==> Crash_Faults/deterministic.tex <==
\section{Deterministic Download with Crash Faults} \label{sec:crash_faults}



In this section, we present deterministic protocols that solve the \download\ problem under the assumption of a synchronous communication network. First, in Section \ref{sec:static}, we show a warm-up deterministic protocol that achieves optimal query complexity, but its time complexity is $O(nf)$, which is inefficient. Then in Section \ref{sec:rapid}, we show how to improve the time complexity by carefully removing some aspects of synchronizations between \peers.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Static Download} 
\label{sec:static}
 
In contrast to the previous section, we consider crash faults instead of byzantine ones. This allows us to circumvent the $\byzfrac n$ lower bound of 
%Theorem {\ref{thm:LB-det-InputDistr}} 
\cite{ABMPRT24}
on the query complexity of \download\, established in \cite{ABMPRT24}. 
We begin by showing a query-optimal deterministic protocol. Later, we present a more complex but also time-optimal protocol.

The static \download\ protocol (Algorithm \ref{alg:static_down}) works as follows.
The execution is partitioned into time segments of $f+1$ rounds each, referred to hereafter as \emph{views}. (In later sections, views may assume other, possibly variable lengths.) Each view $v$ is associated with a publicly known leader denoted $\lead(v)$. We assume throughout that the leader of view $v\geq 0$ is the \peer 
$$
\lead(v) ~=~ v \bmod k.
$$

Each \peer $M$ stores the following local variables.
\begin{itemize}
    \item $\BYZ_M$: The set of crashed \peers that $M$ knows of.
    \item $\view(M)$: $M$'s current view. 
    \item $\indx(M)$: The index of the bit that $M$ currently needs to learn.
   
    \item $\res_M$: $M$'s output. We write $\res_M[i] = \bot$ to indicate that $M$ did not yet assign 
    a value to the $i$'th cell. 
   
\end{itemize}

\paragraph{View $v$ structure.}
% The structure of every view $v$ is as follows.
First, the leader of the view, $\lead(v)$, queries $b_i$ where $i=\indx(\lead(v))$ (we show in Lemma \ref{lem:in_sync} that at any given time, $\indx(M)$ is the same for every \peer $M$). 
Then, for $f+1$ rounds, every \peer $M$ sends $\res_M[\indx(M)]$ (if it knows 

it, i.e., $\res_M[\indx(M)]\neq \bot$) to every other \peer.
After $f+1$ rounds, every \peer $M$ checks its local value $\res_M[\indx(M)]$. If $\res_M[\indx(M)] = \bot$, it concludes that $\lead(v)$ has crashed and adds it to $\BYZ_M$ (and the bit $\indx(M)$ will have to be queried again in the next view, by another leader). Otherwise, it increases $\indx(M)$ by 1. (We show in Lemma \ref{lem:local_sync} that either every \peer $M$ has $\res_M[\indx(M)] = \bot$ or every \peer $M$ has $\res_M[\indx(M)]\in \{0,1\}$.)
Finally, every \peer $M$ enters the next view $v'$ such that $\lead(v') \notin \BYZ_M$.
We remark that once a new bit is learned, and the {\peers} enter the next view, the leader is replaced even if it did not crash. This is done in order to balance the workload over the {\peers}.

See Algorithm \ref{alg:static_down} for the formal code.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
    \caption{Static \download\ (Code for \peer $M$)} 
    \label{alg:static_down}
    \begin{algorithmic}[1]
    \State \textbf{Local variables} 
        \State $\res \gets \emptyset$
        \State $\BYZ \gets \emptyset$
        \State $\indx(M) \gets 1$
        \State $\view(M) \gets 1$
        % \State $j \gets 1$
        \State
        
        \While{$\indx(M) \leq n$}
            \If{$\lead(v) = M$} \Comment{Query Step}
                    \State $\res[\indx(M)] \gets \DataQuery(\indx(M))$
                \EndIf
                \For{$t=1, \dots, f +1$} \Comment{Message Step}
                    % \State 
                     \If{$\res[\indx(M)] \ne \bot$}
                    Send a \view $v$ message
                    $\langle \view\ v, \indx(M), \res[\indx(M)] \rangle$
                    to all \peers.
                    \EndIf
                    \State Receive \view $v$ messages from all other \peers.
                    \If{received a \view $v$ message containing 
                    %$b$ 
                    $\langle i, b\rangle$ from at least one \peer}
                        \State 
                        %$\res[\indx(M)] \gets b$
                        $\res[i] \gets b$
                    \EndIf
                    % \If{received $b$ from at least $f+1$ \peers}
                    %     \State break
                    % \EndIf
                \EndFor
                \If{$\res[\indx(M)] = \bot$} \Comment{View change Step}
                    \State $\BYZ \gets \BYZ \cup \{\lead(v)\}$
                \Else
                    % \If{$\indx(M)=n$} Terminate
                    % \EndIf
                    \State $\indx(M) \gets \indx(M) + 1$
                \EndIf
                \State Let $v' >v$ be the least view such that $\lead(v') \notin \BYZ$ and set $\view(M) \gets v'$
                \label{line:next_view}
        \EndWhile
        %\EndProcedure
        %\Procedure{$\indx(M)=n+1$}{}
        %    \State Terminate
        %\EndProcedure
    \end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Since every view takes exactly $f+1$ rounds, we get the following.
\begin{observation}\label{obs:same_pace}
    Every \peer $M$ is at the same step/round within its current view, $\view(M)$.
\end{observation}

For every view $v$, let $t^s_v$ be the first round a \peer $M$ set $\view(M)=v$ and $t^e_v$ be the first round where a \peer $M$ set $\view(M)=v'$ for $v'>v$. We say that the \peers are \emph{in sync in view $v$} 
if at round $t^s_v$, $\view(M)=v$ and $\indx(M)$ and $\BYZ_M$ are the same for every \peer $M$, and at round $t^e_v$, every \peer enters some view $v'>v$ (it follows from the ensuing analysis that it is the same $v'$ for every \peer). 

When the \peers are in sync in view $v$, we denote by $\indx(v)$ the common value of $\indx(M)$ and by $\BYZ_v$ the common value of $\BYZ_M$ for every \peer $M$.


\begin{lemma} \label{lem:local_sync}
    If the \peers are in sync in view $v$, then after the message step in view $v$, the bit $\indx(v)$ is either downloaded (and known to all {\peers}) or missing (i.e., not known to any of the {\peers}).
\end{lemma}
\begin{proof}
    If every \nonfaulty \peer has $\res[\indx(v)] = \bot$ at the end of view $v$, then $\indx(v)$ is missing. Otherwise, let $M$ be a \nonfaulty \peer with $\res[\indx(v)] = b$ at the end of view $v$. Consider the following cases.

    \inline Case 1 - $M$ first received $b$ at iteration $t<f+1$:
        At the next iteration $t+1$, $M$ sends $\langle \indx(v), b \rangle$ 
        to every other \peer, and since it is not faulty, $\res[\indx(v)] = b$ for every \nonfaulty \peer, so $\indx(v)$ is downloaded after the for loop.
    
    \inline Case 2 - $M$ first received $b$ at iteration $t=f+1$:
        In this case, there exists a chain of \peers $\hat{M}_1, \dots, \hat{M}_{f+1}$ such that $\hat{M}_j$ sends $b$ to $\hat{M}_{j+1}$ on rounds $1 \leq j\leq f$ of the for loop in the message step and $\hat{M}_{f+1}$ sends $b$ to $M$. Since there are $f+1$ \peers in the chain (no duplicates are possible since it would indicate that a crashed \peer sent a message after it crashed), at least one of them is \nonfaulty. Let $\hat{M}$ be the \nonfaulty \peer in the chain. We observe that $\hat{M}$ fulfills the condition of Case 1, so $\indx(v)$ is downloaded after the for loop.
\end{proof}

\begin{corollary}\label{cor:same_local_values}
    If \peers are in sync in view $v$, then they share a common value of their local variables throughout the view.
\end{corollary}
\begin{proof}
    The statement is true by definition at the beginning of the view. The only time the local variables change after the start of the view is during the view change step. At that time, by Lemma \ref{lem:local_sync},
    $\indx(v)$ is either downloaded, in which case every \peer $M$ sets $\indx(M)= \indx(v)+1$, or it is missing, in which case every \peer $M$ adds $\lead(v)$ to $\BYZ_M$. Overall, $\BYZ_M = \BYZ_{M'}$ and $\indx(M)= \indx(M')$ for every pair of \peers $M, M'$.
\end{proof}

\begin{lemma} \label{lem:in_sync}
At every round, the \peers are in sync in some view $v\geq 1$.
\end{lemma}

\begin{proof}
% First, note that the \peers are in sync in view $1$ by the initialization 
Towards contradiction, let $v$ be the first view where the \peers are not in sync in $v$. Hence, on round $t^s_v$ either there exists a \peer $M$ that didn't enter view $v$ or not all \peers have the same values in their local variables (note that for $v=1$, this cannot happen by the initialization values of Algorithm {\ref{alg:static_down}} so, $v\geq 2$).
    
The former cannot happen because by Observation \ref{obs:same_pace}, every \peer enters a new view at the same time, so $M$ must have started some view $\hat{v} \neq v$ at round $t^s_v$. Yet, the \peers were in sync in every view $v'<v$ which means that by Corollary \ref{cor:same_local_values}, in the view prior to $v$, say $v'$, every \peer $M$ had the same value of $\BYZ_M $ meaning that every \peer enters the same view at the end of view $v'$, so $\hat{v} = v$, contradiction. 
    
The latter cannot happen because the local values of \peer $M$ at round $t^s_v$ are the same as the local values at round $t^e_{v'}$ of \peer $M$, where $v'<v$ is the view prior to $v$, for every \peer $M$, and by Corollary \ref{cor:same_local_values} those are the same for every \peer.
\end{proof}

\begin{lemma}
    If the \peers are in sync in view $v$, then when a \peer sets $\res[i] \gets b$, it follows that $b=b_i$.
\end{lemma}
\begin{proof}
    For \peer $M$ to set $\res[i]\gets b$, there must exists a sequence of \peers \- $M_1, M_2, \dots, M_r$ of length $r$ such that $M_r=M$, $M_j$ sent $b$ to $M_{j+1}$ for $j=1,\dots, r-1$ and $M_1$ made a query and received $b$. Since the \peers are in sync, the local $\indx(M)$ of every \peer $M$ is the same and equals $i$, so $M_1$ queried $b_i$, hence $b=b_i$.
    \end{proof}

It follows that if $\res[i] \neq \bot$, then $\res[i] = b_i$.

Note that $\indx(v)\leq \indx(v+1) \leq \indx(v)+1$ and $\indx(1)=1$. 
We get the following corollary by combining Lemmas \ref{lem:local_sync} and \ref{lem:in_sync}.
\begin{corollary} \label{cor:downloaded_or_missing}
    After every view $v$, $\indx(v)$ is either downloaded or missing.
\end{corollary}

\begin{lemma} \label{lem:nonfaulty_leader}
    For view $v>0$, if $\lead(v)$ is \nonfaulty, then $\indx(v)$ is downloaded at the end of $v$.
\end{lemma} 

\begin{proof}
    At the beginning of view $v$, $\lead(v)$ queries the bit $\indx(v)$ and sends it to every other \peer. Subsequently, every \nonfaulty \peer sets $\res[\indx(v)] \gets b_{\indx(v)}$ so $\indx(v)$ is downloaded.
\end{proof}

By Lemma \ref{lem:nonfaulty_leader} and Corollary \ref{cor:downloaded_or_missing}, we get the following corollary.

\begin{corollary} \label{cor:justified_blacklist}
    For view $v>0$, if $\indx(v)$ is missing at the end of view $v$, then $\lead(v)$ crashed, and it is added to $\BYZ$.
\end{corollary}

\inline Correctness: 
By Corollary \ref{cor:downloaded_or_missing}, after every view $v$, $\indx(v)$ is either downloaded or missing. By Corollary \ref{cor:justified_blacklist}, if $\indx(v)$ is missing, $\lead(v)$ will be added to $\BYZ$ and will never be the leader again. Hence, there are at most $f$ views $v$ at the end of which $\indx(v)$ is missing. at the end. So, after $n+f$ views, all $n$ bits are downloaded.

\inline Complexity:
Call a view \emph{good} (respectively, \emph{bad}) if $\indx(v)$ is downloaded (resp., missing) by the end of it. 
As explained above, the protocol is finished after at most $n+f$ views, $n$ of which are good, and at most $f$ are bad. Each view $v$ incurs one query and takes $O(f)$ rounds. 

By Lemma \ref{lem:nonfaulty_leader}, the good views are led by \nonfaulty \peers in a round-robin fashion. Hence, every \nonfaulty \peer leads at most $\frac{n}{\goodfrac k}$ good views. By Corollary \ref{cor:justified_blacklist},  the bad views are led by crashed \peers, and each such \peer may be a leader of a bad view at most once (since it is subsequently added to $\BYZ$). Generally, a \peer may be a leader at most $\frac{n}{\goodfrac k}$ times.
Hence, the query complexity is $\Query=O(\frac{n}{\goodfrac k})$, and the time complexity is $\Time= O(nf)$. Moreover, since at every iteration of the for loop every {\peer} sends a message, we get a message complexity of $\Message = O(k^2\cdot f\cdot n)$.

\begin{theorem} \label{thm:sync_static_download}
In the synchronous model with $f\le \byzfrac k$ crash faults where $\byzfrac<1$, there is a deterministic protocol that solves \download\ with $\Query = O(\frac{n}{\goodfrac k})$, $\Time = O(nf)$ and $\Message = O(k^2\cdot f n)$.
\end{theorem}

%david{Each of the four subsections should end with a summarizing theorem like the above.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Rapid Download } 
\label{sec:rapid}

Algorithm \ref{alg:static_down} has optimal query complexity and is simple but is not optimal in time complexity.
It uses a standard technique of sending a value for $f+1$ rounds, ensuring that by the end, either every {\peer} commits the value or none of them do.
This creates a bottleneck that prolongs the execution time of the protocol.
It is worth noting that it was shown in {\cite{FLP}} that in the presence of $f$ crash faults, agreement must take at least $f+1$ rounds. Hence, shortening the length of a view inevitably breaks the property described above.
%The bottleneck in terms of times lies with each view taking $O(f)$ rounds.
We present the following improved algorithm to overcome this bottleneck.
%
%Each \peer stores the following local variables.
%\begin{itemize}
%    \item $\BYZ_M$: The set of crashed \peers $M$ knows of.
%    \item $\view(M)$: $M$'s current view.
%    \item $\indx(M)$: The index of the current bit $M$ needs to learn.
%%%%%%    % \item $i_M$: The smallest index of a bit $M$ doesn't know.
%    \item $\res_M$: $M$'s output.
%\end{itemize}
%The algorithm works as follows. 
%

Like Algorithm \ref{alg:static_down}, the algorithm is partitioned into views 
and uses the notations $\view$, $\lead$, $\BYZ$, and $\indx$ as defined earlier. 
Unlike that algorithm, in which views were changed automatically on fixed rounds, here the {\peers} need to initiate a \say{view change} process, and send \say{view change} messages in order to change the view. 
This allows us to shorten the span of every view from $f+1$ rounds to just two rounds, but it also brings about some difficulties in coordination. Specifically, Algorithm {\ref{alg:static_down}} ensures that at any given time, every {\peer} has the same values in its local variables as every other {\peer}, while in Algorithm {\ref{alg:rapid_down}}, different {\peers} can be in different views at the same time, with a different set of known bits and a different set of known crashed {\peers}. 
Because of that, it is necessary to carefully construct the transition process between views, referred to as \emph{view change}, so that the most and least advanced {\peers} are at most one bit index apart (in terms of their local variable {$\indx(M)$}) and that progress is always guaranteed.

A view $v$ starts after the leader of that view, $\lead(v)$, first receives messages of type \say{view change} at some round $t$.

We proceed with a more detailed description of the algorithm.

\paragraph{Leader instructions in view $v$.}
The \peer $M$ becomes a leader when it receives a \viewchange $v$ message for the first time. It then starts executing the leader instructions described above.

When view $v$ starts at the beginning of some round $t$ (the first round when $\lead(v)$ received \viewchange $v$ messages), $\lead(v)$ picks the \viewchange $v$ message with the highest index $i$ amongst those received at the end of round $t-1$ and queries the bit $b_i$. Then, $\lead(v)$ sends a \view $v$ message$\langle \view, v, i, b_i \rangle$ to every other \peer, \emph{twice}, in two consecutive rounds.

\paragraph{Instructions when receiving a \view $v$ message.}
When a non-leader \peer $M$ in view $v$ receives a \view $v$ message $\langle \view, v, i, b \rangle$, it first updates its local $\view(M)$ variable to $v$ if $v\geq \view(M)$. Then, it updates its local $\indx(M)$ variable to $i$ if $i\geq \indx(M)$. Finally, it stores $b$ in $\res_M[i]$. If the message is the second one received from $\lead(v)$, then $M$ increases $\indx(M)$ by 1 and moves to the next `available' view 
$v'$ (i.e., such that $\lead(v')$ is not in the list $\BYZ_M$ of crashed \peers),
by a view change process detailed below. 



If a non-leader \peer $M$ has $\view(M)=v$ (and is not during a view change) and didn't receive a \view $v$ message from $\lead(v)$, it adds $\lead(v)$ to $\BYZ_M$ and initiates a view change process as before.

\paragraph{View change instructions.}
When a \peer $M$ initiates a \viewchange $v$ process at time $t$, it invokes Procedure \viewchange in which it sends the next leader, $\lead(v)$, a \viewchange $v$ message %containing $\indx(M)$ 
$\langle \viewchange\ v, \indx(M) \rangle$.
%In the next round, $M$ enters view $v$ and follows the above instructions. 
Subsequently, at time $t+1$, $M$ enters an Idle state for one time step (until time $t+2$) while it waits for $\lead(v)$ to receive the previously sent \viewchange $v$ message, in which it does not expect to receive {\view} messages from any leader (during that time step, $\lead(v)$ collects \viewchange $v$ messages and starts sending {\view} messages that will be received at time $t+2$). Note that if a {\view} $v'\geq v$ message is received during the Idle state (at time $t+1$), then $M$ leaves the Idle state early and proceeds as described above
(this may happen if some other {\peer} $M'$ has initiated a view change one round earlier than $M$). Hence, at the end of a \viewchange $v$, $M$ enters view $v$ only if $v > \view(M)$.

\paragraph{Remarks.}
We make two remarks about the possible behavior of the algorithm. First, note that it is possible for $M=\lead(v)$ to get {\viewchange} messages in more than one round. In particular, suppose that in some view $v'$, $\lead(v')$ is faulty, and in its first round (time $t$) it informs the {\peer} $M'$ but does not inform $M''$. At time $t+1$, $M''$ marks $\lead(v')$ faulty and invokes \viewchange, so the next leader, $M=\lead(v)$, gets its message at time $t+2$. At the same time ($t+2$), $M'$ realizes that $\lead(v')$ has failed, and invokes \viewchange, so $M$ gets its message at time $t+3$. Note that this example also shows that a view might be of different lengths for different \peers.

Second, note that it is possible that $M=\lead(v)$ will receive {\viewchange} messages with different indices $i,i+1$, in consecutive rounds. A possible scenario where this might happen is as follows. Suppose the previous leader, $M'=\lead(v')$, failed in its second transmission round, sending the {\view} message to $M''$ but not to $M'''$. then $M''$, having received the message twice, invokes {\viewchange} $v$ with index $\indx(M'')+1$, while $M'''$, having missed the second message, invokes {\viewchange} $v$ with index $\indx(M''')$. Since $\indx(M'') = \indx(M''')=i$, $M$ will get {\viewchange} messages with $i$ and $i+1$. In this case, $M$ will work on $i+1$, and the bit $b_i$ will never be transmitted again. This is fine, however, since this bit has already been sent to everyone by the previous leader, $M'$, on its first transmission round.

\commentstart
%
%david{I hid the figures; they were mainly meant to clarify the notation for us, and we do not have a high-quality version.}
%
Figures {\ref{fig:execution_timeline_nofaults}} and {\ref{fig:execution_timeline_with_faults}} illustrate two example executions. The first involves \nonfaulty leaders and shows the ``normal" way the execution should look like. The second involves a faulty leader, crashing on its first transmission round, and illustrates how {\peers} change views adaptively and handle crashes.

%
% FIGURES HERE
%
\def\FIGURES{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{execution_timeline_no-faults.jpeg}
    \caption{Execution timeline with \nonfaulty leaders}
    \label{fig:execution_timeline_nofaults}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{execution_timeline_with faults.jpeg}
    \caption{Execution timeline with faulty leaders}
    \label{fig:execution_timeline_with_faults}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
} %FIGURES
\FIGURES
\commentend

See Algorithm {\ref{alg:rapid_down}} for the formal code. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[htb]
    \caption{Rapid \download\ (Code for \peer $M$)}
    \label{alg:rapid_down}
    \small
    \begin{algorithmic}[1]
    \State \textbf{Local variables} 
        \State $\BYZ$, initially $\emptyset$ \Comment{The set of crashed \peers $M$ recognized}
        % \State $C \gets 0$
        \State $\view(M)$, initially 1 \Comment{This is the current view of $M$}
        \State $\indx(M)$, initially 1 \Comment{The index of the current bit $M$ needs to learn}
        % \State $i$, initially 1 \Comment{The smallest index of a bit $M$ doesn't know.}
        \State $\res[i]$, $i\in \{1,\dots, n\}$, initially $\bot$ \Comment{Output array}
        
        % \Procedure{entering view $v$}{}
        %     \For{$j=1,2$}
        %         \If{$\lead(v) = M$} 
        %             \If{$\res[i] = \bot$}
        %                 \State $\res[i] \gets \DataQuery(i)$
        %             \EndIf
        %             \State Send \view $v$ message containing $\langle i, \res[i] \rangle$ to every \peer.
        %         \EndIf
        %         \State Receive $(i', b)$ from $\lead(v)$
        %         \If{didn't receive a message from $\lead(v)$}
        %             \State $\BYZ \gets \BYZ \cup \lead(v)$
        %         \ElsIf{$i'>i$} 
        %             \State 
                
        %         \EndIf
        %     \EndFor
        % \EndProcedure
        
        \State \Comment{Instructions for view $v$ leader}
        \Upon{receiving \viewchange $v$ message for the first time 
        }
        
        \Comment{View changes to $v$, $M=\lead(v)$ becomes leader}
        
        \State From all messages $\langle \viewchange, v, i\rangle$ received in the current round, select  the highest  index $i$.
        \If{$\indx(M) < i$}

\State $\indx(M) \gets i$
        \EndIf
        \If{$\res[\indx(M)] = \bot$}
                \State $\res[\indx(M)] \gets \DataQuery(\indx(M))$ 
            \EndIf
        \For{$j=1,2$}
            
            \State Send a \view $v$ message %containing $\langle \indx(M), \res[\indx(M)] \rangle$
            $\langle \view\ v, \indx(M), \res[\indx(M)] \rangle$ to every \peer.
        \EndFor
        \EndUpon
        \State \Comment{\peer instructions in view $v$}
        \Upon{receiving a  message 
        %$\langle \view~ v, i, b \rangle$}
        $\langle \view~ v, i, b_i \rangle$}
    
            \If{$v \geq \view(M)$}
                
                \State $\view(M)\gets v$
                \If{$i \geq \indx(M)$}
                    \State$\indx(M) \gets i$
                \EndIf
                \State $\res[i] \gets b$
            \EndIf
            
           
            \If{this is the second \view $v$ message received}
                \State $\indx(M)\gets \indx(M)+1$
            \State Invoke Procedure $\viewchange$.
            \EndIf
        \EndUpon
        \State
        \Upon{not receiving a message from 
        %$\lead(v)$
        $\lead(\view(M))$ for an entire round 
        %that is not a view change round 
        and 
        %$\Idle=$ False
        not idle}
        
            \State 
            %$\BYZ \gets \BYZ \cup \lead(v)$
            $\BYZ \gets \BYZ \cup \{\lead(\view(M))\}$
            
           
            \State Invoke Procedure $\viewchange$.
        \EndUpon
        
        
        
        \State \Comment{view change instructions}
        
        
        \Procedure{\viewchange}{}
        %changing $\view(M)$ to $v$
            \State Let $v' >\view(M)$ be the least view such that $\lead(v') \notin \BYZ$.
            \State Send a {\viewchange} message %containing $\indx(M)$
            $\langle \viewchange\ v', {\indx(M)} \rangle$ to $\lead(v')$
            \State Stay idle for one round. 
            \State \textbf{if} $v\geq \view(M)$ \textbf{then} $\view(M) \gets v'$.
            % \If{$\lead(v') = M$}
            %     \State 
            % \EndIf
        \EndProcedure
        
    \end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph*{Analysis.}
We now establish correctness and analyze the algorithm's complexity.




We say that a view $v$ is \emph{\nonfaulty} if $\lead(v)$ is \nonfaulty during view $v$ and \emph{faulty} otherwise.

\begin{lemma}\label{lem:leader_active}
    If, at any time $t$, some \peer $M$ has $\view(M)=v$, then either $\lead(v)$ also has $\view(\lead(v)) = v$, or $\lead(v)$ has crashed.
\end{lemma}
\begin{proof}
A \peer $M$ enters view $v$ either by performing a view change or by getting a \view $v$ message from $\lead(v)$. In the former case, $\lead(v)$ has not yet entered view $v$. After the view change, both $M$ and $\lead(v)$ enter view $v$ and by the structure of the view they both remain in view $v$ for one or two more rounds, until either $\lead(v)$ crashes or two \view $v$ messages are received, which results in the end of view $v$. In the latter case, $\lead(v)$ has already entered view $v$ and $M$ receives the first \view $v$ message (out of two) and enters view $v$. Both $M$ and $\lead(v)$ remain in view $v$ for one more round, until the second message is received or $\lead(v)$ crashes.
\end{proof}

\begin{lemma} \label{lem:BYZ_justified}
If a \peer $M$ adds $\lead(v)$ to $\BYZ_M$, then $\lead(v)$ has crashed.
\end{lemma}
\begin{proof}
A \peer $M$ adds $\lead(v)$ to $\BYZ_M$ if'f $\view(M)=v$ and $M$ didn't receive a \view $v$ message from $\lead(v)$ (at some round other than the idle round).

By Lemma \ref{lem:leader_active}, it cannot be the case that $\lead(v)$ is in a different view, and since it hasn't sent a \view $v$ message while in view $v$, it must have crashed.
\end{proof}
\begin{lemma} \label{lem:sync_view}
    At the beginning of the second round of a \nonfaulty view $v$, every \peer $M$ has $\view(M)= v$.
\end{lemma}
\begin{proof}
During the first round of a \nonfaulty view $v$, $\lead(v)$ sends a \view $v$ message to every \peer. Subsequently, every \peer that is in a previous view advances to view $v$ (while every other \peer remains unaffected). Therefore, after the first round of view $v$, $\view(M)\geq v$ for every \peer $M$. Assume towards contradiction that there exists some \peer $M'$ such that $\view(M') > v$ at the beginning of the second round of view $v$. For that to be the case, $M'$ must have added $\lead(v)$ to $\BYZ_{M'}$, in contradiction to Lemma \ref{lem:BYZ_justified} and the fact that view $v$ is \nonfaulty.
\end{proof}

\begin{lemma}\label{lem:confirmed_bit}
For every two nonfaulty \peers $M, M'$ and index $i$, if $i < \indx(M)$ then $\res_{M'}[i] = b_i$. 
%for every \nonfaulty \peer $M'$
\end{lemma}
\begin{proof}
Let $M$ be a \nonfaulty \peer. 
%We note that for $\indx(M)$ to increase
For every $i < \indx(M)$, let $M_i$ be the first \nonfaulty {\peer} to set $\indx(M_i) > i$. Since $M_i$ is the first to increase $\indx(M_i)$ above $i$, it must be the case that 
%for every $i < \indx(M)$, $M$
$M_i$ received two \view $v$ messages from some leader, 
%$\langle \view~ v, i, b \rangle$
$\langle \view~ v, i, b_i \rangle$.
Since 
%$M$ 
$M_i$ received two messages, every \nonfaulty \peer $M'$ must have received at least one such message, and subsequently set $\res_{M'}[i]=b_i$.
\end{proof}



Let $\minbit(t) = \min_{\mbox{\footnotesize \peers~} M}\{\indx(M)~\mbox{at round}~t\}$. 
\begin{lemma}\label{lem:min_bit_increase}
For every view $v\geq 1$, $\minbit(t^e_v)\geq \minbit(t^s_v) +1$.
\end{lemma}
\begin{proof}
By Lemma \ref{lem:sync_view}, at the beginning of the second round of view $v$ every \peer $M$ has $\view(M)= v$. Hence, when view $v$ finishes, at round $t^e_v$, every \peer $M$ has $\indx(M)\geq \indx(\lead(v))+1 \geq \minbit(t^s_v)+1$. Hence, the Lemma follows.
\end{proof}
\begin{lemma} \label{lem:time_fast_rapid}
    After $n+f$ views, every \peer knows the entire input $\invec$
\end{lemma}
\begin{proof}
    By Lemma \ref{lem:min_bit_increase}, $\minbit$ increases after every \nonfaulty view. Out of $n+f$ views, at most $f$ might be faulty, by Lemma \ref{lem:BYZ_justified} and the fact that once a \peer $M$ adds another \peer $M'$ to $\BYZ_M$ it will not enter any view $v$ where $\lead(v) = M'$. Therefore, after $n+f$ views, $\indx(M) \geq n+1$ for every \peer $M$. By Lemma \ref{lem:confirmed_bit}, this means that $\res_M[i] = b_i$ for every $1\leq i\leq n$ and \peer $M$.
\end{proof}
\begin{theorem} \label{thm:sync_rapid_download}
In the synchronous  model with $f\le \byzfrac k$ crash faults where $\byzfrac<1$, there is a deterministic protocol that solves \download\ with $\Query = O(\frac{n}{\goodfrac k})$, $\Time = O(n+f)$ and $\Message = O\left(k\cdot (n+f)\right)$.
\end{theorem}
\begin{proof}
By Lemma \ref{lem:time_fast_rapid}, after $n+f$ views, every \peer knows the entire input. A view takes at most two rounds; hence, the time complexity is $\Time=O(n+f)$. By Lemma \ref{lem:min_bit_increase}, every \nonfaulty view increases $\minbit$ by at least 1, so after $n$ \nonfaulty views the protocol terminates. Because we use round robin order for leaders, every \nonfaulty \peer is the leader of at most $n/\goodfrac k$ views. Hence, the query complexity is $\Query=\frac{n}{\goodfrac k}$. Moreover, since every non leader {\peer} communicates only with its current leader and every leader communicates with every other {\peer}, the number of messages per round is $O(k)$, so
%and the message complexity is 
$\Message = O(k(n+f))$.
\end{proof}

==> Query-optimal_Download/correctness.tex <==
\paragraph{Correctness.}  Let $P_j  =  1 - \left(1 - \frac{1}{\goodfrac k}\right)^{2^j}$ be the probability that when flipping $2^j$ independent random coins, each with bias $\frac{1}{\goodfrac k}$ toward head, at least one turns heads. The following technical lemma provides upper and lower bounds on $P_j$.
\begin{lemma} \label{lem: bound Pj - 2}
    For $j \in [f,\lg (\goodfrac k) - \lg \lg n ]$, $P_j \in \left(\frac{2^j}{\goodfrac k} \left(1 -\frac{1}{2\lg n}\right), \frac{2^j}{\goodfrac k}\right)$. 
\end{lemma}
\begin{proof}
The binomial expansion of $(1 - \varepsilon)^m$ yields the bounds
$1 - m\varepsilon  <  (1-\varepsilon)^m  <  1 - m\varepsilon + \frac{m(m-1)}{2}\varepsilon^2$. Setting $\varepsilon=1/\gamma k$ and $m=2^j$, we get 
$1-2^j/\gamma k < (1-1/\gamma k)^{2^j} < 1-2^j/\gamma k + 2^j(2^j-1)/(2(\gamma k)^2)$, or
$$\frac{2^j}{\gamma k} ~>~ P_j ~>~ \frac{2^j}{\gamma k} - \frac{2^j(2^j-1)}{2(\gamma k)^2}
~>~ \frac{2^j}{\gamma k}\left(1 - \frac{1}{2} \frac{2^j}{\gamma k}\right)
~>~ \frac{2^j}{\gamma k}\left(1 - \frac{1}{2\lg n}\right)
~,$$
where the last inequality follows from the assumption that $2^j < \gamma k/\lg n$.
\end{proof}

To prove the correctness of the algorithm, we need to show that all \nonfaulty \peers $M$ compute $\invec^M = \invec$ correctly with high probability. This is shown by inductively proving that, for any \nonfaulty \peer $M$ and any bit $i$, $1 \le i \le n$, $b_i^M = b_i$ with high probability. The induction is on $i$ for a fixed \nonfaulty \peer $M$. We prove the following two invariant statements inductively.


\begin{description}
    \item[Blacklisting Statements ($BL_i$).]  All \peers blacklisted by some \nonfaulty \peer $M$ until the end of the $i$-th epoch (i.e., the \ith iteration of the outer {\tt for} loop, line~\ref{for:outer}) of Algorithm~\ref{alg:improved}) are indeed Byzantine, with high probability. For convenience, $BL_0$ refers to the empty blacklist before the execution enters the loop and is clearly true.
    
    To capture the inner {\tt for} loop as well (line~\ref{for:inner} of Algorithm~\ref{alg:improved}), we use $BL_{i,j}$, $1 \le i < n$ and  $j \in [f, \lceil{\lg (\gamma k)-\lg \lg n} \rceil ]$ to refer to the statement that all \peers blacklisted by some \nonfaulty \peer $M$ until the end of the \jth inner {\tt for} loop of the $(i+1)$-st epoch are indeed Byzantine, with high probability. For convenience, we sometimes use $BL_{i, f-1}$ to refer to $BL_i$. Also, note that $BL_{i,\lceil{\lg (\gamma k)-\lg \lg n} \rceil}$ implies $BL_{i+1}$.
    
    
    \item[Correctness Statement ($C_i$).] All \nonfaulty \peers have executed the first $i$ epochs correctly, with high probability, i.e., $b_{i'}^M = b_{i'}$ for all $1 \le i' \le i$ and all \nonfaulty \peers $M$. Again, $C_0$ refers to the execution being vacuously correct before any bit is processed by the \peers. Furthermore, $C_{i,j}$, $1\le i<n$ and $j \in [f, \lceil{\lg (\gamma k)-\lg \lg n} \rceil ]$,  refers to the following statement at the end of iteration $j$ in epoch $(i+1)$: for all non-faulty peers $M$, $b_{i'}^M = b_{i'}$ for all $1 \le i' \le i$ and $b_{i+1}^M = b_{i+1}$ for all \nonfaulty \peers that have set their respective $I_{voted}$ bit to 1, with high probability. For convenience, we sometimes use $C_{i, f-1}$ to refer to $C_i$. Also, note that $C_{i,\lceil{\lg (\gamma k)-\lg \lg n} \rceil}$ implies $C_{i+1}$.
\end{description}


Observe that \peer $M$ performs a query if (a) it is the first round of that particular epoch and it has obtained ``heads'', or (b) it is round $j > f$, it is the first time $M$ has drawn ``heads'', and $COUNT_i^b \ge \nu 2^j$ for \emph{both} $b=0$ and $b=1$.

The basis for the induction is provided by the statements $BL_0$ and $C_0$, which are both true. The inductive step is given by the following lemma.
\begin{lemma} \label{lem:correctness}
    Consider some epoch $i \in [1,n]$ and assume that conditions $BL_{i-1}$ and $C_{i-1}$ hold at the start of epoch $i$. For any fixed $c \ge 1$, there is a suitably small fixed choice for the constant $\delta$ such that the statements $BL_i$ and $C_i$ hold with probability at least $1 - \frac{1}{n^{c + 1}}$ at the end of the epoch $i$. 
\end{lemma}
\begin{proof}
Fix $c \ge 1$. To prove the claim, we show that $BL_{i,j}$ and $C_{i,j}$ hold for all rounds $j \in [f, \lceil{\lg (\gamma k)-\lg\lg n} \rceil]$. By the inductive hypothesis, $BL_{i, f-1} = BL_{i-1}$ and $C_{i, f-1} = C_{i-1}$ hold. For the sake of contradiction, suppose statement $C_i$ does not hold, and let $j^*$ be the first round $j$ in epoch $i$ when statement $C_{i-1,j}$ is false, namely, some \peer\ $M$ tosses heads and goes on to set its $I_{voted}$ bit to 1, but incorrectly assigns $b^M_i = 1-b_i$. Since $j^*$ is the first such occurrence of incorrect behavior, $BL_{i-1,j^*-1}$ and $C_{i-1,j^*-1}$ are true. If $j^* = f$, then $M$ will explicitly query the bit, so $b_{i}^M = b_{i}$, a contradiction. So, we focus on the case where $j^* > f$.

Without loss of generality, let $b_i = 0$. We claim that the number of votes received by $M$ in favor of $b_i = 0$ will be at least  $\nu \cdot 2^{j^*} =2^{j^*-2}$ with  probability at least $1 - \frac{1}{n^c}$. Since $BL_{i-1,j^*-1}$ and $C_{i-1,j^*-1}$ are true, all \nonfaulty \peers that tossed heads in earlier rounds $j < j^*$ would have correctly voted for $b_i = 0$. To establish the required contradiction, we show that the number of such votes is at least $\nu \cdot 2^{j^*} = 2^{j^*-2}$. Let $G_{old}$ be the set of votes received by $M$ from \nonfaulty \peers in epoch $i$ during rounds $j$ for $j \le j^*-2$ (if such rounds exist). Let $G_{recent}$ be the set of votes received by $M$ from \nonfaulty \peers in round $j' = j^*-1$; we know this round exists as $j^*>f$. Our goal is to show that $X = G_{old} \cup G_{recent}$ has cardinality $|X| \ge 2^{j^*-2}$ with high probability. Let $G$ denote the set of all \nonfaulty \peers; $|G| \ge \goodfrac k$. Note that for every \peer in $G \setminus G_{old}$, the probability of joining $G_{recent}$ is $P_{j'} = P_{j^*-1}$ by Lemma {\ref{lem: bound Pj - 2}}, so the expected size of $X$ is
$$\Exp[|X|] ~\ge~ |G| \cdot P_{j^*-1} ~\ge~ \gamma k \cdot \frac{2^{j^*-1}}{k\gamma} \left(1 -\frac{1}{2\lg n}\right) ~=~ 2^{j^*-1} \left(1 -\frac{1}{2\lg n}\right) ~\ge~ 0.9\cdot 2^{j^*-1},$$
for sufficiently large $n$ (say, $n\geq 32$).
Thus, applying Chernoff bound, we get
\begin{eqnarray*}
\Pr[|X| &<& 2^{j^*-2}] ~=~ \Pr\left[|X| < 0.5\cdot 2^{j^*-1}\right] 
~\le~ \Pr\big[|X| < (1-4/9) \Exp[|X|]\big]
\\
&<& e^{-\frac{(4/9)^2}{2} \Exp[|X|]} 
~\le~ e^{-\frac{(4/9)^2}{2} \cdot 0.9\cdot 2^{j^*-1}}
~\le~ e^{-\frac{4}{45}\cdot 2^f}
~=~ e^{-\frac{4}{45}\cdot 2^{\delta+\lg\lg n}}
~=~ e^{-\frac{4}{45}\cdot 2^\delta \cdot \lg n}
\\
&< & n^{-\frac{4}{45}\cdot 2^\delta}
~< ~ \frac{1}{n^{c+2}},
\end{eqnarray*}
where the last inequality holds when $\delta \ge \lg (45(c+2)) - 2$).


Thus, the number of votes received by $M$ for the correct bit value (0, as per our assumption wlog) must be at least $\nu \cdot 2^{j^*}$ relying on the fact that by the inductive assumption $BL_{i-1,j^*-1}$, no \nonfaulty \peer was added to $B$. From the else part (see line \ref{line: else_part} of Algorithm~\ref{alg:improved}), if both bit values received $\nu \cdot 2^j$ votes (or more), then $M$ will query bit $i$ and this will ensure $C_{i-1, j^*}$. On the other hand, if the number of votes for bit value 1 is less than $\nu 2^{j^*}$, then, $M$ will vote for 0, which will be the correct bit. Thus, the contradiction is established, thereby implying $C_i$ with probability at least $1 - \frac{1}{n^{c + 1}}$ (applying the union bound over all peers $M$).


If $C_i$ holds, then all other \nonfaulty \peers $M' \ne M$ also vote correctly for $0$, so $M$ will not blacklist any of them. This implies that the invariant $BL_i$ also holds.
\end{proof}



Applying Lemma~\ref{lem:correctness} and taking the union bound over all $n$ epochs, we get the following corollary.
\begin{corollary}
    For $\delta$ fixed as in Lemma~\ref{lem:correctness}, Algorithm~\ref{alg:improved} ensures that all \peers $M$ correctly compute $\invec^M = \invec$ with probability at least $1 - \frac{1}{n^c}$.
\end{corollary}

==> Query-optimal_Download/description.tex <==
Our algorithm runs in $n$ \emph{epochs}. For $1 \leq i \leq n$, a non-faulty peer $M$ dedicates the \ith epoch to learning the \ith input bit. Furthermore, each epoch $i$ is divided into \emph{rounds}. During each round $j$ of the epoch $i$, $M$ attempts to learn the \ith input bit $x_i$ in one of two ways:
\begin{enumerate}
    \item[(i)]  based on messages received from the other peers in earlier rounds, or

    \item[(ii)] by querying the source directly (which happens with gradually increasing probability).
\end{enumerate}
$M$ relies on the messages of its peers for learning $x_i = b$ in round $j$ only if the number of peers who sent it the value $b$ exceeds a specified threshold (depending on $j$) \emph{and} the number of peers who sent it the value $(1 - b)$ is below that threshold. If $M$ fails to learn the bit in round $j$, then it proceeds to round $(j + 1)$, in which it doubles its probability of querying. This is repeated until $M$ successfully learns $x_i$. (Note that a head is always thrown when $2^j$ exceeds $\frac{\goodfrac k}{\lg{n}}$.


Once $M$ learns $x_i$, it broadcasts it and blacklists any peers who send contradictory values. In subsequent rounds, $M$ never relies on bits sent by blacklisted peers. See Algorithm~\ref{alg:improved} for the pseudocode. Note that in each epoch $i$, $M$ learns the value of the \ith bit either by \emph{gossip learning} (i.e., receiving messages with a decisive majority, in line \ref{l:gossip learning} of the algorithm) or by \emph{query learning} (in line \ref{l:query learning}). We name the epoch accordingly as a \emph{gossip} epoch or as a \emph{query} epoch. Furthermore, in every epoch $i$, $M$ performs a ``learning step'' in \emph{exactly one} round, hereafter referred to as the \emph{learning round} of epoch $i$ and denoted $\ell(i)$.

==> Query-optimal_Download/main.tex <==
\section{Query-optimal \download} \label{sec: optimal_time_P2P}





In this section, we show how to optimize the query complexity of \download\ up to a factor of $\log{n}$, achieving $\Query  =  \optqexact  =  \optqtilde$ for any $\byzfrac < 1$. This provides an improvement over the best previously known results for \download~\cite{ABMPRT24}, which either guaranteed a query complexity of $\Query = \tilde{O}\left(\frac{n}{\goodfrac k} + \sqrt{n}\right)$ or imposed the additional restriction of $\byzfrac < \frac{1}{3}$.


The algorithm described next works under the assumption that $2\goodfrac k > 2^\delta \cdot \lg^2{n}$, for some constant $\delta$.\footnote{For any positive real number $x$, we use the notation $\lg{x}$ to denote $\log_2{x}$.}  Note that, for smaller values of $k$, the desired bound of $\optqtilde$ on the query complexity holds trivially: when $k  \leq  \left(\frac{2^{\delta}}{2\goodfrac}\right) \cdot \lg^2{n}$, this bound is $\optqtilde = \tilde{O}(n)$, which is attainable by the trivial algorithm where every peer queries the entire input vector.



\input{Query-optimal Download/description}

\input{Query-optimal Download/pseudocode}

\input{Query-optimal Download/correctness}

\input{Query-optimal Download/query_complexity}



Each epoch lasts $O(\lg{k})$ phases, so the time complexity is $O(n\lg{k})$. Each \peer sends at most $n$ bits to each of the other machines, so the total number of messages sent is $O(nk^2)$. Thus, we have the following theorem.
\begin{theorem} \label{thm:opt-alg-p2p}
    In the synchronous point-to-point model with Byzantine failures, there is a randomized algorithm for \download\ such that with high probability, $\Query = \optqexact$, $\Time = O(n\log{k})$, and $\Message = O(nk^2)$. Moreover, it only requires messages of size $O(1)$.
\end{theorem}

==> Query-optimal_Download/pseudocode.tex <==
\begin{algorithm}
\caption{Resilient \download\ for any fixed known $\byzfrac<1$; code for \peer $M$} \label{alg:improved}
    
    \begin{algorithmic}[1]
        \State $B \gets \emptyset$ \Comment{Set of blacklisted \peers}
        \For{$i$ from 1 to $n$} \label{for:outer} \Comment{Epoch $i$ deals with input bit $x_i$} 

            \State $I_{voted} \gets 0$ \Comment{Indicator of learning the $i$-th bit and voting on it}
            \State $COUNT^0_i \gets 0$; $COUNT^1_i \gets 0$; \Comment{Counters for the number of \peers that voted 0/1 for bit $i$}
            \State $f \gets\lceil{\delta + \lg \lg n}\rceil$; \Comment{See Lemmas~\ref{lem:correctness} and \ref{lem:complexity} for the choice of the constant $\delta$. } \label{lno:constant}
            \For{$j$ from $f$ to $\lceil{\lg (\gamma k)-\lg \lg n} \rceil $} 
            \label{for:inner}
                \If{$I_{voted}=0$ ($M$ has not voted for bit $i$ yet)}
                        \If{$COUNT^{1-b}_i< \nu \cdot 2^{j}$ for $\mbox{$\nu=1/4$ and}$ for some $b \in \{0,1\}$ AND $(j \neq f)$ }
                   \label{l:insufficient_opposition}   \State $b_i^M \gets b$ 
                    \label{l:gossip learning}               \Comment{Perform a “gossip learning” step}
                      \State Broadcast a vote $\langle M,i,b_i^M=b \rangle$\; \Comment{$M$ and $i$ are implicit}
                       \State Set $I_{voted}\gets 1$
                        \Else
                \If{$j = \lceil {\lg (\gamma k-\lg \lg n}\rceil$} 
                \State Set coinflip to heads
                \Else\label{line: else_part}
                    \State Toss $2^j$ independent Coins with bias $1/\gamma k$ towards heads.
                    \State Let $S_{i,j}$ be the number of Coins that turned heads.
                    Set coinflip to heads if $S_{i,j} \ge 1$.
                    \label{lno:toss}
                \EndIf
                    \If{heads} \Comment{Perform a ``query learning" step}
                            \State  $b_i^M \leftarrow b \leftarrow query(i)$; \label{l:query learning} \Comment{$M$ learns $b^M_i=b$ by query}
                        \State Broadcast a vote $\langle M,i,b_i^M=b \rangle$\; \Comment{$M$ and $i$ are implicit}
                        \State Set $I_{voted}\gets 1$
                        \EndIf
                        \EndIf
                         \State Receive messages from other \peers.
                         \For{$b \in \{0,1\}$}
                        \State $COUNT^b_i \gets |\{M' \not\in B \mid M ~\hbox{received message~}\langle M',i,b_i^{M'}=b \rangle ~\hbox{during epoch $i$}\}|$
                        \\
                        \Comment{count voters for $b \in \{0,1\}$; ignore peers
                        blacklisted in earlier epochs}
                	\EndFor
                \EndIf
                \If{$I_{voted}=1$} \Comment{Including the case when $I_{voted}$ changed during the current phase}
                	\State $B\leftarrow B ~ \cup \{M' \mid \hbox{$M'$ sent message with~} b^{M'}_i \ne b^M_i\}$ \Comment{peers with  contradictory vote}
                \EndIf
            \EndFor
        \EndFor
    \end{algorithmic}
\end{algorithm}

==> Query-optimal_Download/query_complexity.tex <==
\paragraph{Query complexity analysis}  In the absence of Byzantine peers, the total number of (necessary) queries is $O(n)$, so the average cost per \peer is clearly $\Query = O\left(\frac{n}{\goodfrac k}\right)$. The reason for the additional wasteful queries is two-fold. First, the fact that the algorithm is randomized and must succeed in learning all bits with high probability requires some redundancy in querying. Second, Byzantine \peers spread fake information, forcing \nonfaulty \peers to perform queries to blacklist the culprits and clarify the true values of $\invec$.


Let $\randvec(M)$ denote the sequence of independent random coins flipped by \peer $M$ during execution (each with a bias of $\frac{1}{\goodfrac k}$ towards heads). For notational convenience, we will often write $\randvec$ \st{$(M)$} to mean $\randvec(M)$, when the underlying peer $M$ is clear from the context. Let $\randvec_{i,j}$ denote the subsequence of $\randvec$ that was drawn at the beginning of round $j$ of the epoch $i$, and let $\randvec_i$ denote the subsequence of $\randvec$ that was drawn during the entire epoch $i$. Respectively, let $R = \modof{\randvec}$, $R_i = \modof{\randvec_i}$ and $R_{i,j} = \modof{\randvec_{i,j}}$.


The variable $S_{i, j}$ used in the algorithm denotes the number of coins of $\randvec_{i,j}$ that turned heads. Similarly, let $S_i$ denote the number of coins of $\randvec_i$ that turned heads.
\begin{lemma} \label{lem:complexity}
    For any fixed $c' \ge 1$, there is a suitably small fixed choice for the constant $\delta$ such that Algorithm~\ref{alg:improved} has query complexity $\Query = \optqexact$ with probability $1 - \frac{1}{n^{c'}}$.
\end{lemma}
\begin{proof}
    Throughout the proof, we consider a non-faulty peer $M$.

    For every $1\le i\le n$, let $B(i)$ denote the number of \peers that were blacklisted by $M$ in epoch $i$ and let $C(i)$ denote the number of queries performed by $M$ in epoch $i$. (Note that $C(i)$ is 0 if $i$ is a \emph{gossip epoch} and 1 if $i$ is a \emph{query epoch}.)

    %Note that in every epoch $i$, $M$ performs a ``learning step'' in \emph{exactly one} round, hereafter referred to as the \emph{learning round} of $i$ and denoted $\ell(i)$.
    
    As $C(i)=0$ for a gossip epoch $i$, the total cost of gossip epochs is
    \begin{equation} \label{eq:Cgossip}
        C^{gossip} ~=~ \sum_{\mbox{\footnotesize gossip}~i} C^{gossip}(i) ~=~ 0.
    \end{equation}
    Hence, we only need to analyze query epochs. We bound the number of queries in these epochs by first bounding the number of random coins flipped in these epochs.
    
    Consider such an epoch $i$, with learning round $\ell = \ell(i)$. There are two cases. The first is when $\ell = f$. In this case, perhaps no faulty \peers were blacklisted, so $B(i)\ge 0$ and the number of random Coins flipped in this epoch is $R_i = R_{i,f} = 2^f$.
    
    The second case is when $\ell > f$. The fact that $M$ had to query in round $\ell$ implies that gossip learning was not possible, so both $COUNT^0_i \ge \nu 2^j = 2^{\ell-2}$ and $COUNT^1_i\ge 2^{\ell-2}$. This, in turn, implies that the number of faulty \peers that $M$ gets to blacklist in this epoch is $B(i) \ge 2^{\ell-2}$. On the other hand, the number of Coins used during this epoch is $R_i = \sum_{j=f}^\ell R_{i,j} = 2^{\ell+1}-2^f$.
    
    Combining both cases, we get that for every epoch $i$, $B(i) \ge (R_i-2^f)/8$. Summing over all $i$, we get that
    \begin{equation*}
        \beta k ~\ge~ B ~=~ \sum_i B(i) ~\ge~ \sum_i \frac{R_i-2^f}{8} ~=~ \frac{R-2^fn}{8}~.
    \end{equation*}
    Rewriting, and recalling that $f=\lceil{\delta + \lg \lg n}\rceil$, we get
    \begin{equation} \label{eq:bound R}
        n\cdot 2^\delta\lg n ~\le~ R ~\le~ 8\beta k + 2^f n~\le~ 8\beta k + n \cdot 2^\delta \lg{n}\text{,}
    \end{equation}
    where the first inequality follows from the fact that in every epoch $i$, $R_i\ge R_{i,f} \ge 2^\delta\lg n$.
    
    Note that $C(i)\le S_i$ for every $i$, hence
    \begin{equation} \label{eq:Cquery}
        C^{query} ~=~ \sum_{\mbox{\footnotesize query}~i} C(i) \le \sum_{\mbox{\footnotesize query}~i} S_i ~=~ S.
    \end{equation}
    Recalling that $\randvec$ is a sequence of $R$ independent Bernoulli variables with probability $\frac{1}{\goodfrac k}$ for heads, we have that $\Exp[S]  =  \frac{R}{\goodfrac k}$, and applying Chernoff bound we get
    \begin{equation} \label{eq: S vs R}
        \Pr[S > 2R/\gamma k] ~=~ \Pr[S > 2 \Exp[S]] ~\le~ e^{-\Exp[S]/3} ~=~ e^{-R/3\gamma k} ~\le~ e^{-n 2^\delta\lg n/3\gamma k} ~\le~ \frac{1}{n^{c'}}~\text{,}
    \end{equation}
    where the penultimate inequality relies on the left side of Eq. \eqref{eq:bound R} and the last one holds when $\delta \ge \lg (3\gamma c')$, also relying on the assumption that $k \le n$. Combining Equations \eqref{eq:Cquery}, \eqref{eq: S vs R}, and the right side of \eqref{eq:bound R}, we get that with probability at least $1 - \frac{1}{n^{c'}}$,
    \begin{equation} \label{eq:Cquery-sum}
        C^{query} ~\le~ S ~\le~ \frac{2R}{\gamma k} ~\le~ \frac{2(8\beta k + cn\lg n)}{\gamma k}  ~=~  \optqexact.
    \end{equation}
    Finally, the lemma follows by Equations {\eqref{eq:Cgossip}} and {\eqref{eq:Cquery-sum}}.
\end{proof}

==> lower_bound_-_single_round.tex <==
\section{A Lower Bound} \label{section-lower-bounds}





Having established the existence of a query-optimal algorithm for the \download\ problem with an arbitrary bound $\byzfrac<1$ on the fraction of faulty peers, we turn to the issue of time complexity and derive faster \download\ algorithms. In this section, we ask whether a single round algorithm exists (assuming arbitrarily large messages can be sent in a single round), other than the trivial algorithm where every \peer queries every bit. We show that this is impossible: if we insist on a single round algorithm, then every \peer must query all bits.



\paragraph{Notations and Terminology.}  Let $V$ be a set of $n$ \peers in the network. Recall that $\beta$ is the maximum allowed fraction of Byzantine \peers in any execution and $\gamma$ is the minimum fraction of \nonfaulty \peers ($\beta+\gamma=1$). In this section we assume, for simplicity, that $n$ is odd, and fix $\beta=(n-1)/2n$, i.e., we assume that at most $(n-1)/2$ \peers might fail in any execution.
Let the input vector be denoted by $\invec  =  \left\{b_1, b_2, \ldots, b_n\right\}$.


For positive integers $q$ and $t$, let $\mathcal{A}(q, t)$ be the class of all randomized Monte-Carlo algorithms with query complexity at most $q$ and time complexity at most $t$. (Note that this class encompasses the class of deterministic algorithms as well.) We fix an algorithm $A \in \mathcal{A}(n - 1, 1)$, and from this point on we make our arguments with respect to this algorithm $A$.


In every execution of algorithm $A$, the first (and only) round starts (at the beginning of the query sub-round) with each \peer $v\in V$ making some random coin flips and generating a random bit string $R_v$. The resulting \emph{random profile} of the execution is $R = \langle R_1, \ldots, R_k \rangle$, the collection of random strings selected by the $k$ peers. Based on its random bit string $R_v$, each \peer $v$ computes a list of indices that it queries (unless it fails).



\begin{defn} \label{def: weak adversary}
    A \emph{weak} adversary is one that fixes its adversarial strategy \emph{before} the start of the execution. This strategy is composed of selecting a set $\byz\subseteq V$ of \peers to fail in the execution, subject to the constraint that $|\byz| \leq \beta n$, and a set of rules dictating the actions of the \peers in $\byz$, including the messages that are to be sent by each Byzantine \peer. 
\end{defn}

\begin{defn} \label{def: execution}
    We define an \emph{execution} of the algorithm $A$ as the 3-tuple $\EXEC = (\invec, \byz, R)$, where $\invec$ is the input vector (which can be chosen by the adversary), $\byz$ is the set of Byzantine \peers selected by the adversary, and  $R$ is the random profile selected by the \peers. We denote $\good=V\setminus \byz$. We say that the execution $\EXEC(\invec,\byz,R)$ \emph{succeeds} if all \peers acquire all $n$ bits. 
\end{defn}



A key observation is that for every non-faulty peer $v$, the list of queried indices is determined by its random bit string $R_v$, and is independent of $\invec$ and $\byz$. Hence, the random profile $R$ fully determines the list of queried indices of every \peer.


We refer to a random profile $R$ for which some \peer fails to query the $i^{\text{th}}$ input bit as an \emph{$i$-defective} random profile. Let
\begin{eqnarray*}
\RR &=& \{ R \mid R ~\mbox{is a random profile of some execution of}~ A \},
\\
\RR_i &=& \{ R \in \RR \mid R ~\mbox{is}~ i\mbox{-defective} \}.
\end{eqnarray*}

Note that each random profile $R$ may occur with a different probability $p_R$, such that $\sum_{R\in\RR} p_R = 1$.
For any subset $\RR' \subseteq \RR$, let
$p(\RR)= \sum_{R\in\RR'} p_R$.

\begin{lemma} \label{lemma-BE-ell}
    For the algorithm $A$, there is an index $\ell=\ell(A)$, $1\le\ell\le n$, such that $p(\RR_\ell) ~\ge~ 1-e^{-1}$.
\end{lemma}

\begin{proof}
Let $\EXSET$ denote the set of executions of algorithm $A$. For each \peer $v$, let $\EXSET_v$ be the set of executions in which $v$ does not fail, and let $r=|\EXSET_v|$. 
For $i \in [1, n]$, let $r_v(i)$ denote the number of executions in $\EXSET_v$ in which $v$ does not query $i$, and let $p_v(i) = r_v(i)/r$ be the probability that $v$ does not query $i$.


Note that by definition of the class $\mathcal{A}(n-1,1)$, $\sum_i r(v,i) \ge r$, because for every execution $e\in \EXSET_v$ there is at least one bit $i$ that $v$ does not query in $e$, or in other words, every such execution is counted in one of the counters $r(v,i)$. It follows that
\begin{equation} \label{eq:P ge 1}
    \sum_{i = 1}^n p_v(i) ~=~ \frac{\sum_i r(v,i)}{r} ~\geq~  1 ~~~~~~ \mbox{for every \peer}~ v.
\end{equation}
The adversary can calculate the probabilities $p_v(i)$
for every \peer $v$. Subsequently, it can compute for every index $i$ the probability that \emph{no} \peer skips $i$, namely, 
\begin{equation} \label{eq:qi formula}
    q(i) ~=~ \prod_{v} (1 - p_v(i)),
\end{equation}
and pick $\ell$ to be the index minimizing $q(i)$. We claim that for such an index $\ell$, $p(\RR_\ell) ~\ge~ 1-e^{-1}$. To see this, note that it can be shown that under constraints {\eqref{eq:P ge 1}} and {\eqref{eq:qi formula}}, $q(i)$ is maximized when $p_v(i) = \frac{1}{n}$ for every $v$ and every $i$. Then
\begin{equation*}
    q(i) ~=~ \prod_{v} (1 - p_v(i))   ~\leq~   \left(1 - \frac{1}{n}\right)^{n}
    ~<~   e^{-1}~.
\end{equation*}
As $p[\RR_\ell] = 1-q(\ell)$, the lemma follows.
\end{proof}



For an $\ell$-defective random profile $R\in \RR_\ell$, denote by $v(R)$ the \emph{defective} \peer $v$ that does not query the $\ell^{\text{th}}$ input bit. (In case more than one such \peer exists, we pick one arbitrarily.)
\begin{lemma}
    There is a (non-adaptive) adversarial strategy that foils Algorithm $A$ with probability at least $(1-e^{-1})/4$.
\end{lemma}
\begin{proof}
The proof is by an \emph{indistinguishability} argument. 
Let $\ell=\ell(A)$ be the index whose existence is asserted by Lemma \ref{lemma-BE-ell}.
For any input vector $\invec$, let $\invX{\invec}$ be another $n$-bit vector that's identical to
$\invec$ except for the $\ell^{\text{th}}$ bit, which is inverted in $\invX{\invec}$. The adversary fixes an arbitrary input vector $\invec_0$ in which $b_\ell=0$,
and sets the vector $\invec_1$ to be  $\invX{\invec_0}$.
%
The adversarial strategy is to select the set $\byz$ of $(n-1)/2$ Byzantine \peers uniformly at random from the collection $\BB$ of all $n\choose (n-1)/2$ possible choices. For any input vector $\invec$, the Byzantine peers are instructed to execute the same protocol as the \nonfaulty \peers, but on the vector $\invX{\invec}$. In other words, in executions on $\invec_0$, the Byzantine \peers will run algorithm $A$ on $\invec_1$, and vice versa.

We are interested in subsets of the set $\EXSET$ of executions of algorithm $A$. In particular, for any specific input $\invec'$ and subsets $\RR'\subseteq\RR$ and $\BB' \subseteq \BB$, let $\EXSET(\invec',\RR',\BB')$ denote the set of all executions $\EXEC(\invec,\byz,R)$ where $\invec=\invec'$, $\byz\in\BB'$ and $R\in \RR'$.

Hereafter, we only consider executions where the random profile $R$ is $\ell$-defective and $v(R)\not\in\byz$ for the set $\byz$ selected by the adversary, i.e.,
where $R$ belongs to the set
$$\hRR(\byz) ~=~ \{ R \mid R\in\RR_\ell,~~~v(R)\not\in\byz\}.$$
Note that since the set $\byz$ is selected by the adversary uniformly at random and independently of $R$, $\Pr[v(R)\not\in\byz] > 1/2$, hence, applying Lemma \ref{lemma-BE-ell}, we get that for any $\byz\in\BB$,
\begin{equation}
\label{eq:p-hRR-byz}
p(\hRR(\byz)) ~>~ (1-e^{-1})/2.
\end{equation}
For the rest of the proof, we concentrate on executions from
$\EXSET(\invec_0,\BB,\hRR(\byz))$ and $\EXSET(\invec_1,\BB,\hRR(\byz))$, and aim to show that in at least one of the two sets, the executions fail with constant probability. 

For $\byz\in \BB$ and random profile $R$, let
$\invB_R = V\setminus(\byz\cup\{v(R)\})$.  

\begin{claim}
\label{cl:one of two fails}
Consider some $\byz\in\BB$ and $R\in\hRR(\byz)$. Then the defective \peer $v=v(R)$ identifies the bit $b_\ell$ in the same way in the executions $\EXEC(\invec_0,\byz,R)$ and $\EXEC(\invec_1,\invB,R)$, namely, at least one of the two executions fails. Formally, noting that both
$\Pr[\EXEC(\invec_0,\byz,R) ~\text{fails}]$ and $\Pr[\EXEC(\invec_1,\invB,R) ~\text{fails}]$ are  0 or 1, the claim implies that 
$$\Pr[\EXEC(\invec_0,\byz,R) ~\text{fails}] + 
\Pr[\EXEC(\invec_1,\invB,R) ~\text{fails}] \ge 1.$$
\end{claim}
\begin{proof}
Let $\goodv$ (respectively, $\byzv$) be the set of messages sent from peers in the set $\good - \lbrace v \rbrace$ (resp., $\byz$) to $v$ in execution $\EXEC(\invec_0,\byz,R)$, and let
%\begin{equation*}
    $\allv  ~=~  \goodv \cup \byzv$.
%\end{equation*}
Define $\goodpv$, $\byzpv$ and $\allpv$ analogously
%to $\goodv$, $\byzv$ and $\allv$
w.r.t. the execution $\EXEC(\invec_1,\invB,R)$.
The key observation here is that
$$\goodv = \byzpv ~~~~~ \mbox{ and }~~~~~ \byzv = \goodpv.$$ 
This implies that
\begin{equation}
\label{eq:same messages}
    \allpv  ~=~  \goodpv  \cup  \byzpv  ~=~  \byzv \cup \goodv  ~=~  \allv\text{.}
\end{equation}
That is, the set of messages received by $v$ is identical in both executions.

Since $v$ sees the same inputs and the same incoming messages in both of these executions, it follows that it will identify the bit $b_\ell$ in the same way in both executions. But whichever identification it makes, in one of the two executions this identification is false, hence that execution fails.
\end{proof}

For a given $\byz$, let $p_{fail}^0(\byz,\RR')$ denote the probability that the execution $\EXEC(\invec_0,\byz,R)$ fails, conditioned on $R\in \RR'$, and let $p_{fail}^1(\invB,\RR')$ denote the probability that the execution $\EXEC(\invec_1,\invB,R)$ fails, conditioned on $R\in \RR'$. Then
\begin{eqnarray}
p_{fail}^0(\byz,\RR') 
&=& \Pr[\EXEC(\invec_0,\byz,R)~\mbox{fails} \mid R\in\RR']
~=~ \frac{\Pr[\EXEC(\invec_0,\byz,R)~\mbox{fails} ~\wedge~ R\in\RR']}{\Pr[R\in\RR']}
\nonumber
\\
&=& \frac{1}{p(\RR')} \cdot\sum_{R\in\RR'} p_R\cdot\Pr[\EXEC(\invec_0,\byz,R)~\mbox{fails}].
\label{eq:def fail}
\end{eqnarray}


Hence, for any $\byz\in\BB$, applying \eqref{eq:def fail} to $\RR$ and noting that $p(\RR)=1$,
\begin{eqnarray*}
p_{fail}^0(\byz,\RR) &=&
\sum_{R\in\RR} p_R\cdot\Pr[\EXEC(\invec_0,\byz,R)~\mbox{fails}]
~\ge~ \sum_{R\in\hRR(\byz)} p_R\cdot\Pr[\EXEC(\invec_0,\byz,R)~\mbox{fails}].
\end{eqnarray*}
Similarly, we get that
$$p_{fail}^1(\invB,\RR) ~\ge~
\sum_{R\in\hRR(\byz)} p_R\cdot\Pr[\EXEC(\invec_1,\invB,R)~\mbox{fails}].$$
Combining the last two inequalities with Claim \ref{cl:one of two fails} and Eq. \eqref{eq:p-hRR-byz}, we get that for any $\byz\in\BB$,
\begin{eqnarray}
p_{fail}^0(\byz,\RR) + p_{fail}^1(\invB,\RR) &\ge&
\sum_{R\in\hRR(\byz)} p_R\cdot(\Pr[\EXEC(\invec_0,\byz,R) + \Pr[\EXEC(\invec_1,\invB,R))
\nonumber
\\
&\ge& \sum_{R\in\hRR(\byz)} p_R ~=~ p(\hRR(\byz)) ~>~ (1-e^{-1})/2.
\label{eq:pfail 0+1}
\end{eqnarray}
For $i=0,1$, let $p_{fail}^i = \Pr[\EXEC(\invec_i,\byz,R)~\mbox{fails} \mid \byz\in\BB,~ R\in \RR]$. Then
\begin{eqnarray*}
p_{fail}^0 &=& \frac{1}{|\BB|} \sum_{\byz\in\BB} p_{fail}^0(\byz,\RR),
\\
p_{fail}^1 &=& \frac{1}{|\BB|} \sum_{\byz\in\BB} p_{fail}^1(\byz,\RR)
~=~ \frac{1}{|\BB|} \sum_{\byz\in\BB} p_{fail}^1(\invB,\RR),
\end{eqnarray*}
where the last equality follows from observing that, since $((\byz)^{\textsf{inv}})^{\textsf{inv}} = \byz$, and since the probability is taken over all $\byz\in\BB$, $p_{fail}^1$ also equals the probability that the execution $\EXEC(\invec_1,\byz,R)$ fails, conditioned on $\byz\in\BB$ and $R\in \RR$.
It follows from Eq. \eqref{eq:pfail 0+1} that
$$p_{fail}^0 + p_{fail}^1 
~=~ \frac{1}{|\BB|} \sum_{\byz\in\BB} (p_{fail}^0(\byz,\RR) + p_{fail}^1(\invB,\RR))
~>~ \frac{1}{|\BB|} \sum_{\byz\in\BB} (1-e^{-1})/2
~=~ (1-e^{-1})/2.$$
Without loss of generality, $p_{fail}^0 \ge (1-e^{-1})/4$. This implies that the algorithm fails on the input vector $\invec_0$ with this probability. The lemma follows.
\end{proof}



\begin{theorem}
    Consider an $n$-\peer system with external data, for odd $n$, and let the fraction of Byzantine \peers be bounded above by $\beta = (n-1)/2n$. For every algorithm $A \in \mathcal{A}(n - 1, 1)$, there is an adversarial strategy such that $A$ fails to learn all the input bits with probability at least $(1-e^{-1})/4$. The lower bound holds even in the broadcast communication model.
\end{theorem}

==> table_-_summary_of_all_the_results.tex <==
\begin{table}[!t]
\centering \footnotesize
\begin{tabular}
{|P{3.68cm}|P{2.15cm}|P{2.90cm}|P{2.59cm}|P{2.9cm}|}

\hline
\multicolumn{5}{|c|} {\bf Comparison of the Existing and Developed Results for Byzantine Fault}\\
\hline
  {\bf Adversary}&{\bf Theorem} &{\bf Query} & {\bf Time} & {\bf Message Size}\\
\hline

                 & \cite{ABMPRT24} & $\tilde{O}(n/k + \sqrt{n})$  & $O(n)$        & $O(\log n)$\\
Fixed Byzantine  & \cite{ABMPRT24}\# & $\tilde{O}(n/k)$             & $O(n)$        & $O(\log n)$\\
                 & Thm~\ref{thm:opt-alg-p2p} & $\tilde{O}(n/k)$     & $O(n\log k)$  & $O(1)$\\
\hline

Dynamic Byzantine   &Thm~\ref{thm:2-round}         &$\tilde{O}( n/ k + \sqrt{n})$     &$2$ & $\tilde{O}(n/ k + \sqrt{n})$\\
           &Thm~\ref{thm:fast_expected_optimal}   &$\tilde{O}( n/ k)$*      &$O(\log n)$ & $\tilde{O}(n)$\\
\hline

Dynamic Byzantine &Cor~\ref{cor:broadcast-time-query} &$O(n/k)$* &$O(\log n)$& $O(n/k)$\\
and Broadcast     &Thm~\ref{thm:broadcast_whp}    &$O(n/k)$   & $O(\log^2 n)$ &$\tilde{O}(n/k)$\\

\hline
\end{tabular}
\caption{Our main results (with $\beta$ treated as {\it any} positive constant in $[0,1)$). Here, $^\ast$ denotes results that only hold in expectation, and \# denotes that $\beta<1/3$. }\label{tbl: comparative_analysis}
\end{table}
\begin{table}[!t]
\centering \footnotesize
\begin{tabular}
{|P{3.68cm}|P{2.15cm}|P{2.90cm}|P{2.59cm}|P{2.9cm}|}

\hline
\multicolumn{5}{|c|} {\bf Deterministic Protocol with Crash Fault}\\
\hline
  {\bf Model}&{\bf Theorem} &{\bf Query} & {\bf Time} & {\bf Message Size}\\
\hline

Synchronous &Thm~\ref{thm:sync_rapid_download}\# &$O(n/k)$ &$O(n+k)$& $O(\log n)$\\
\hline

Asynchronous &Thm~\ref{thm:async_single_crash} &$O(n/k)$ & $\tilde{O}\left(\frac{n}{k}\right)$& $O(\log n)$\\
             &Thm~\ref{thm:async_multi_crash} & $O(n/k)$ &$O(n)$& $O(\log n)$\\

\hline
\end{tabular}
\caption{Our main results for $\beta<1$ in the crash fault setting for synchronous and asynchronous model. \# denotes that $\beta \leq 1/ k$.}\label{tbl: sync_results}
\end{table}
